Robust 1-bit Compressed Sensing with Iterative Hard Thresholding

In 1-bit compressed sensing, the aim is to estimate a $k$-sparse unit vector $x\in S^{n-1}$ within an $\epsilon$ error (in $\ell_2$) from minimal number of linear measurements that are quantized to just their signs, i.e., from measurements of the form $y = \mathrm{Sign}(\langle a, x\rangle).$ In this paper, we study a noisy version where a fraction of the measurements can be flipped, potentially by an adversary. In particular, we analyze the Binary Iterative Hard Thresholding (BIHT) algorithm, a proximal gradient descent on a properly defined loss function used for 1-bit compressed sensing, in this noisy setting. It is known from recent results that, with $\tilde{O}(\frac{k}{\epsilon})$ noiseless measurements, BIHT provides an estimate within $\epsilon$ error. This result is optimal and universal, meaning one set of measurements work for all sparse vectors. In this paper, we show that BIHT also provides better results than all known methods for the noisy setting. We show that when up to $\tau$-fraction of the sign measurements are incorrect (adversarial error), with the same number of measurements as before, BIHT agnostically provides an estimate of $x$ within an $\tilde{O}(\epsilon+\tau)$ error, maintaining the universality of measurements. This establishes stability of iterative hard thresholding in the presence of measurement error. To obtain the result, we use the restricted approximate invertibility of Gaussian matrices, as well as a tight analysis of the high-dimensional geometry of the adversarially corrupted measurements.

==> notation-15-2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Notation and Preliminaries} %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\label{section:|>notation+prelim}    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\COMMENT{Evidently, this section needs some work..}

%Define the universal constants
%\ToDo{Fill these in.}
%%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
%%\(  \aC, \bC, \cC, \cX{1}, \cX{2}, \cX{3} > 0  \)
%%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%as
%%|>>|===========================================================================================|>>|
%\begin{subequations}
%\label{eqn:univ-consts}
%\begin{gather}
%\label{eqn:univ-consts:1}
%  \text{\ToDo{Fill these in.}}
%\end{gather}
%\end{subequations}
%%|<<|===========================================================================================|<<|

Throughout this work, the parameters \(  \k, \n \in \Z_{+}  \) are taken to satisfy,
\(  \n \geq 2\k  \).

Unless specified otherwise, the map
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \f[\Mat{M}] : \R^{\n} \to \BinarySet^{\m}  \)
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
denotes an arbitrary function satisfying
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \DistH{\f( \Vec{x} )}{\Sign( \Mat{M} \Vec{x} )} \leq \tauX \m  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
where \(  \Mat{M} = ( \Vec{M}\VL{1} \;\cdots\; \Vec{M}\VL{\m} )^{\T} \in \R^{\m \times \n}  \).
%
As the specific choice of \(  \Mat{M} \in \R^{\m \times \n}  \)
will in general be clear from context, the matrix will be omitted from the notation,
writing instead: \(  \f = \f[\Mat{M}]  \).
%
In the context of this work, \(  \f  \) represents an arbitrary noise function which may be chosen by the adversary.


Define
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \h, \hf{}{} : \R^{\n} \times \R^{\n} \to \R^{\n}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%|>>|===========================================================================================|>>|
\begin{subequations}
\label{eqn:h:def}
\begin{gather}
  \label{eqn:h:def:h_A}
  \h( \Vec{x}, \Vec{y} )
  =
  \frac{\sqrt{2\pi}}{\m}
  \Mat{\AM}^{\T}
  \cdot \frac{1}{2}
  \bigl( \Sign( \Mat{\AM} \Vec{x} ) - \Sign( \Mat{\AM} \Vec{y} ) \bigr)
  =
  \frac{\sqrt{2\pi}}{\m}
  \sum_{\iIx=1}^{\m}
  \Vec{\AV}\VL{\iIx}
  \cdot \frac{1}{2}
  \bigl( \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{x} \rangle )
         -
         \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{y} \rangle )
  \bigr)
  ,\\ \label{eqn:h:def:h_fA}
  \hf{\Vec{x}}{\Vec{y}}
  =
  \frac{\sqrt{2\pi}}{\m}
  \Mat{\AM}^{\T}
  \cdot \frac{1}{2}
  \bigl( \fAx - \Sign( \Mat{\AM} \Vec{y} ) \bigr)
  =
  \frac{\sqrt{2\pi}}{\m}
  \sum_{\iIx=1}^{\m}
  \Vec{\AV}\VL{\iIx}
  \cdot \frac{1}{2}
  \bigl( \fAix
         -
         \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{y} \rangle )
  \bigr)
,\end{gather}
\end{subequations}
%|<<|===========================================================================================|<<|
and for \(  \JX \subseteq [\n]  \), let
\(  \h[\JX], \hf[\JX]{}{} : \R^{\n} \times \R^{\n} \to \R^{\n}  \)
denote
%|>>|===========================================================================================|>>|
\begin{subequations}
\label{eqn:h_J:def}
\begin{gather}
  \label{eqn:h:def:h_AJ}
  \h[\JX]( \Vec{x}, \Vec{y} ) =
  \ThresholdSet'{\Supp( \Vec{x} ) \cup \Supp( \Vec{y} ) \cup \JX}( \h( \Vec{x}, \Vec{y} ) )
  ,\\ \label{eqn:h:def:h_fAJ}
  \hf[\JX]{\Vec{x}}{\Vec{y}} =
  \ThresholdSet'{\Supp( \Vec{x} ) \cup \Supp( \Vec{y} ) \cup \JX}( \hf{\Vec{x}}{\Vec{y}} )
.\end{gather}
\end{subequations}
%|<<|===========================================================================================|<<|

Note that
%|>>|===========================================================================================|>>|
\begin{gather*}
  \frac{1}{2}
  \bigl( \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{x} \rangle )
         -
         \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{y} \rangle )
  \bigr)
  =
  \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{x} \rangle )
  \cdot
  \I( \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{x} \rangle )
      \neq \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{y} \rangle ) )
%,\end{gather*}
%%|<<|===========================================================================================|<<|
%and likewise,
%%|>>|===========================================================================================|>>|
%\begin{gather*}
  \\
  \frac{1}{2}
  \bigl( \fAix
         -
         \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{y} \rangle )
  \bigr)
  =
  -\Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{y} \rangle )
  \cdot
  \I( \fAix \neq \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{y} \rangle ) )
.\end{gather*}
%|<<|===========================================================================================|<<|
%
It follows that
%|>>|===========================================================================================|>>|
\begin{subequations}
\label{eqn:notation:h:def-alt}
\begin{gather}
  \label{eqn:notation:hA:def-alt}
  \h( \Vec{x}, \Vec{y} )
  =
  \frac{\sqrt{2\pi}}{\m}
  \sum_{\iIx=1}^{\m}
  \Vec{\AV}\VL{\iIx}
  \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{x} \rangle )
  \cdot
  \I( \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{x} \rangle )
      \neq \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{y} \rangle ) )
  ,\\ \label{eqn:notation:hfA:def-alt}
  \hf{\Vec{x}}{\Vec{y}}
  =
  -\frac{\sqrt{2\pi}}{\m}
  \sum_{\iIx=1}^{\m}
  \Vec{\AV}\VL{\iIx}
  \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{y} \rangle )
  \cdot \I( \fAix \neq \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{y} \rangle ) )
.\end{gather}
\end{subequations}
%|<<|===========================================================================================|<<|

For \(  \Vec{\uX} \in \R^{\n}  \) and \(  \betaX \in [0,\pi]  \), define
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \BallAngular{\betaX}( \Vec{\uX} )
    \defeq \{ \Vec{v} \in \R^{\n} : \DistAngular{\Vec{\uX}}{\Vec{v}} \leq \betaX \}  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|

Given a set of vectors, \(  \Set{U} \subseteq \R^{\n}  \),
and a coordinate subset, \(  \JX \subseteq [\n]  \), write
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \ThresholdSet{\JX}[\Set{U}]
    \defeq \{ \ThresholdSet{\JX}( \Vec{u} ) : \Vec{u} \in \Set{U} \}
    \subseteq \R^{\n}  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|

For \(  \JX \subseteq [\n]  \), the restriction of \(  \Vec{u} \in \R^{\n}  \) to the entries
indexed by \(  \JX  \) is denoted by
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Restriction{\Vec{u}}{\JX} \in \R^{| \JX |}  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
\begin{comment}
Extending this notation, for a set of vectors,
\(  \Set{U} = \{ \Vec{u}\VL{1}, \dots, \Vec{u}\VL{\m} \}  \),
the restriction of each element in \(  \Set{U}  \) to the entries indexed by \(  \JX  \)
is written as
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Restriction{\Set{U}}{\JX}
    = \{ \Restriction{\Vec{u}\VL{1}}{\JX}, \dots, \Restriction{\Vec{u}\VL{\m}}{\JX} \}
    \subseteq \R^{| \JX |}  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
\end{comment}

For notational simplicity, the parameter \(  \tauX  \) is assumed to satisfy
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \tauX \m \in \Z_{+}  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
Note that we need not consider \(  \tauX = 0  \) since \cite{matsumoto2022binary}
already established the result under noiseless conditions.

The universal constants,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \aC, \bC, \cX{1}, \cX{2}, \cX{3}, \cX{4}, \cX{} > 0  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
are fixed as:
%|>>|===========================================================================================|>>|
\begin{subequations}
\label{eqn:universal-constants}
\begin{align}
  &
  \aC = \aValue,
  &&
  \bC \lesssim \bCValue,
  \\
  &
  \cX{1} = \cXOneValue \in ( \cXOneValueX, \cXOneValueXX ),
  &&
  \cX{2} = \cXTwoValue \in ( \cXTwoValueX, \cXTwoValueXX ),
  \\
  &
  \cX{3} = \cXThreeValue \in ( \cXThreeValueX, \cXThreeValueXX ),
  &&
  \cX{4} = \cXFourValue \in ( \cXFourValueX, \cXFourValueXX ),
  \\
  &
  \cX{} = 4 \left( \cX{1} + \sqrt{\cX{1}^{2} + \cX{2}} \right)^{2}
        \in ( \cValue, \cValueXX ).
%  &
%  \aC = \aValue,
%  &&
%  \bC \lesssim \bCValue,
%  \\
%  &
%  \cX{1} = \cXOneValue \lesssim \cXOneValueX,
%  &&
%  \cX{2} = \cXTwoValue \lesssim \cXTwoValueX,
%  \\
%  &
%  \cX{3} = \cXThreeValue \lesssim \cXThreeValueX,
%  &&
%  \cX{4} = \cXFourValue \lesssim \cXFourValueX
%  \\
%  &
%  \cX{} = 4 \left( \cC[1] + \sqrt{\cX{1}^{2} + \cX{2} + \cX{3}} \right)^{2} \lesssim \cValue.
\end{align}
\end{subequations}
%|<<|===========================================================================================|<<|

For \(  \deltaX > 0  \), define the map, \(  \mO : \R \to \R  \), by
%|>>|===========================================================================================|>>|
\begin{gather*}
  \mO[\deltaX]
  \defeq
  \frac{\bC}{\deltaX}
  \Log(
    \binom{\n}{\k}^{2}
    \binom{\n}{2\k}
    \left( \frac{12 \bC}{\deltaX} \right)^{2\k}
    \left( \frac{3 \aC}{\rhoX} \right)
  )
  \in
  \BigO(
    \frac{\k}{\deltaX} \Log( \frac{\n}{\deltaX \k} )
    +
    \frac{1}{\deltaX} \Log( \frac{1}{\rhoX} )
  )
.\end{gather*}
%|<<|===========================================================================================|<<|

\begin{algorithm}
\label{alg:biht:normalized}
\caption{Binary iterative hard thresholding (BIHT) algorithm, normalized projections}
%
Set \( \Eta = \sqrt{2\pi} \)\;
%
%\(
%  \Vec{\tilde{x}}^{(0)}
%  =
%  \frac{\Eta}{m}
%  \MeasMat^{\T}
%  \Sgn( \MeasMat \Vec{x} )
%\)\;
%
%\(
%  \Vec{\hat{x}}^{(0)}
%  =
%  \frac
%  {\Threshold{k}( \Vec{\tilde{x}}^{(0)} )}
%  {\left\| \Threshold{k}( \Vec{\tilde{x}}^{(0)} ) \right\|_{2}}
%\)\;
%
\(
  \Vec{\hat{x}}^{(0)}
  \sim
  \SparseSphereSubspace{k}{n}
\)\;
%
\For
{\( \Iter = 1, 2, 3, \dots \)}
{
  \(
    \Vec{\tilde{x}}^{(\Iter)}
    \gets
    \Vec{\hat{x}}^{(\Iter-1)}
    +
    \frac{\eta}{m}
    \MeasMat^{\T}
    \cdot
    \frac{1}{2}
    \left(
      \Sgn{} \big( \MeasMat \Vec{x} \big) - \Sgn{} \big( \MeasMat \Vec{\hat{x}}^{(\Iter-1)} \big)
    \right)
  \)\;
  \(
    \Vec{\hat{x}}^{(\Iter)}
    \gets
    \frac
    {\Threshold{k}(\Vec{\tilde{x}}^{(\Iter)})}
    {\left\| \Threshold{k}(\Vec{\tilde{x}}^{(\Iter)}) \right\|_{2}}
  \)\;
}
\end{algorithm}

==> notation-15-3-a.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Preliminaries}  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\label{section:|>prelim} %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Notations}              %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\label{section:|>prelim|>notations} %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\COMMENT{Evidently, this section needs some work..}

%Define the universal constants
%\ToDo{Fill these in.}
%%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
%%\(  \aC, \bC, \cC, \cX{1}, \cX{2}, \cX{3} > 0  \)
%%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%as
%%|>>|===========================================================================================|>>|
%\begin{subequations}
%\label{eqn:univ-consts}
%\begin{gather}
%\label{eqn:univ-consts:1}
%  \text{\ToDo{Fill these in.}}
%\end{gather}
%\end{subequations}
%%|<<|===========================================================================================|<<|

Throughout this work, the parameters \(  \k, \n \in \Z_{+}  \) are taken to satisfy
\(  \n \geq 2\k  \),
where \(  \k  \) denotes sparsity (i.e., the maximum number of nonzero entries in a vector),
and where \(  \n  \) is the dimension of the signal vectors and measurements.
%
The number of measurements (and rows in the measurement matrix) is denoted by \(  \m \in \Z_{+}  \).
%
For notational simplicity, the parameter \(  \tauX \in (0,1]  \)%
---the fraction of responses that can be corrupted---%
is assumed to satisfy
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \tauX \m \in \Z_{+}  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
This does not forgo generality since \(  \tauX \m  \) can be replaced by
\(  \lceil \tauX \m \rceil  \) throughout the analysis in this manuscript.
%
Note that this work does not consider \(  \tauX = 0  \) since \cite{matsumoto2022binary}
already established the result under noiseless conditions.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\par %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
For the purposes of this discussion, let \(  \Ell, \dX \in \Z_{+}  \),
where \(  \dX \in \Z_{+}  \) specifies an arbitrary dimension.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\par %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
Let \(  \Distr{D}  \) be an arbitrary distribution.
%
Then, \(  \RV{X} \sim \Distr{D}  \) denotes a random variable
which follows the distribution \(  \Distr{D}  \).
%
Similarly, let \(  \Set{S}  \) be an arbitrary set.
%
Then, \(  \RV{X} \sim \Set{S}  \) denotes a random variable
which follows the uniform distribution over \(  \Set{S}  \).
%
The univariate normal distribution with
mean \(  \mu \in \R  \) and variance \(  \sigma^{2} \in \R_{\geq 0}  \)
is denoted by \(  \N( \mu, \sigma^{2} )  \),
while the \(  \dX  \)-variate normal distribution with
mean vector \(  \Vec{\mu} \in \R^{\dX}  \) and
covariance matrix \(  \Mat{\Sigma} \in \R^{\dX \times \dX}  \)
is denoted by \(  \N( \Vec{\mu}, \Mat{\Sigma} )  \).
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\par %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
The \(  \dX  \)-dimensional identity matrix is denoted by \(  \Id{\dX} \in \R^{\dX \times \dX}  \).
%
More generally, matrices are written as capital letters in boldface, upright typeface, e.g.,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Mat{A} \in \R^{\Ell \times \dX}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
with the \(  i\Th  \) rows denoted by, e.g.,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Mat{A}\VL{i} \in \R^{\dX}  \), \(  i \in [\Ell]  \), such that
\(  \Mat{A} = ( \Mat{A}\VL{1} \cdots \Mat{A}\VL{\Ell} )^{\T}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
and with the \(  (i,j)  \)-entries written in italic typeface, e.g.,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Mat*{A}_{i,j} \in \R  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
Nonrandom vectors are written as lowercase letters in boldface, upright typeface, e.g.,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Vec{u} \in \R^{\dX}  \)
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
with the \(  j\Th  \) entries, \(  j \in [\dX]  \), written in italic typeface, e.g.,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Vec*{u}_{j} \in \R  \), such that
\(  \Vec{u} = ( \Vec*{u}_{1}, \dots, \Vec*{u}_{\dX} )  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
Random vectors follow the same convention as nonrandom vectors but with uppercase letters, e.g.,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Vec{Z} = ( \Vec*{Z}_{1}, \dots, \Vec*{Z}_{\dX} ) \sim \N( \Vec{0}, \Id{\dX} )  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
For \(  \JX \subseteq [\dX]  \), the restriction of \(  \Vec{u} \in \R^{\dX}  \) to the entries
indexed by \(  \JX  \) is denoted by
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Restriction{\Vec{u}}{\JX} \in \R^{| \JX |}  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
The support of a vector, \(  \Vec{u} \in \R^{\dX}  \), is denoted by
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Supp( \Vec{u} ) \defeq \{ j \in [\dX] : \Vec*{u}_{j} \neq 0 \} \subseteq [\dX]  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
and the number of nonzero entries in \(  \Vec{u}  \)%
---the \(  \lnorm{0}  \)-``norm'' of \(  \Vec{u}  \)---%
is written as
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \| \Vec{u} \|_{0} \defeq | \Supp( \Vec{u} ) |  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\par %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
The \(  \lnorm{2}  \)-unit sphere in \(  \R^{\dX}  \) is denoted by
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Sphere{\dX} \defeq \{ \Vec{u} \in \R^{\dX} : \| \Vec{u} \|_{2} = 1 \}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
and the set of \(  \k  \)-sparse \(  \dX  \)-dimensional vectors is written as
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \SparseSubspace{\k}{\dX} \defeq \{ \Vec{u} \in \R^{\dX} : \| \Vec{u} \|_{0} \leq \k \}  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
Hence, the set of all \(  \dX  \)-dimensional, \ksparserealunit vectors is denote by
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \SparseSphereSubspace{\k}{\dX} \defeq
    \{ \Vec{u} \in \Sphere{\dX} : \| \Vec{u} \|_{0} \leq \k \}  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
The distance between two points projected onto the \(  \lnorm{2}  \)-unit sphere is specified by
the function
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \DistSOp{\dX} : \R^{\dX} \times \R^{\dX} \to \R_{\geq 0}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
where
%|>>|===========================================================================================|>>|
\begin{gather*}
  \DistS[\dX]{\Vec{u}}{\Vec{v}}
  =
  \begin{cases}
  \left\| \frac{\Vec{u}}{\| \Vec{u} \|_{2}} - \frac{\Vec{v}}{\| \Vec{v} \|_{2}} \right\|_{2},
     &\cIf \Vec{u}, \Vec{v} \neq \Vec{0}, \\
  0, &\cIf \Vec{u} = \Vec{v} = \Vec{0}, \\
  1, &\cOtherwise,
  \end{cases}
\end{gather*}
%|<<|===========================================================================================|<<|
for \(  \Vec{u}, \Vec{v} \in \R^{\dX}  \).
%
The sign function, \(  \Sign. : \R \to \BinarySet  \), follows the convention:
%|>>|===========================================================================================|>>|
\begin{gather*}
  \Sign( a )
  =
  \begin{cases}
   -1, &\cIf a    < 0, \\
  \+1, &\cIf a \geq 0,
  \end{cases}
\end{gather*}
%|<<|===========================================================================================|<<|
where \(  a \in \R  \).
%
This notation extends to vectors as \(  \Sign. : \R^{\dX} \to \BinarySet^{\dX}  \)
by taking the \(  \pm  \)-signs of each entry of a \(  \dX  \)-dimensional vector.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\par %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
This work considers two notions of hard thresholding as means to project points into
the subspace of \(  \Ell  \)-sparse vectors, \(  \SparseSubspace{\Ell}{\dX}  \):
\topk[\(  \Ell  \)] and \ksubset[\(  \Ell  \)] \hardthresholding.
%
These are formalized in the following definitions.
%
%|>>|###########################################################################################|>>|
%|>>|###########################################################################################|>>|
%|>>|###########################################################################################|>>|
\begin{definition}[{\Topk[\(  \Ell  \)] \hardthresholding}]
\label{def:top-k-hard-thresholding}
%
%Let \(  \Vec{u} \in \R^{\dX}  \).
%
The \emph{\topk[\(  \Ell  \)] \hardthresholding operation}, denoted by
\(  \Threshold{\Ell} : \R^{\dX} \to \R^{\dX}  \),
projects a vector \(  \Vec{u} \in \R^{\dX}  \) into \(  \SparseSubspace{\Ell}{\dX}  \)
by retaining only the \(  \Ell  \) largest (in absolute value) entries in \(  \Vec{u}  \)
and setting all other entries to \(  0  \).
%
Note that ``ties'' can be broken arbitrarily.
%
More formally, writing
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Set{U}_{\Ell} = \{ \Vec{u'} \in \R^{\dX} : \| \Vec{u'} \|_{0} = \Ell, \ \Vec*{u'}_{j} \in \{ \Vec*{u}_{j}, 0 \} \ \forall j \in [\dX] \}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
the \topk[\(  \Ell  \)] \hardthresholding operation maps:
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(
  \Vec{u} \mapsto
  \Threshold{\Ell}( \Vec{u} )
  \in \arg\max_{\Vec{u'} \in \Set{U}_{\Ell}} \| \Vec{u'} \|_{1}
\).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
\end{definition}
%|<<|###########################################################################################|<<|
%|<<|###########################################################################################|<<|
%|<<|###########################################################################################|<<|
%
%|>>|###########################################################################################|>>|
%|>>|###########################################################################################|>>|
%|>>|###########################################################################################|>>|
\begin{definition}[{\kSubset[\(  \Ell  \)] \hardthresholding}]
\label{def:k-subset-hard-thresholding}
%
%Let
%%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
%\(  J \subseteq [\dX]  \).
%%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
The \emph{\ksubset \hardthresholding operation}
associated with a coordinate subset \(  J \subseteq [\dX]  \),
denoted by
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \ThresholdSet'{J} : \R^{\dX} \to \R^{\dX}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
takes a vector, \(  \Vec{u} \in \R^{\dX}  \), into \(  \SparseSubspace{|J|}{\dX}  \)
by setting all entries in \(  \Vec{u}  \) indexed by \(  [\dX] \setminus J  \) to \(  0  \).
%
More formally, \(  \ThresholdSet'{J}( \Vec{u} )  \) is the vector whose \(  j\Th  \) entries,
\(  j \in [\dX]  \), are given by
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \ThresholdSet*'{J}( \Vec{u} )_{j} = \Vec*{u}_{j} \cdot \I( j \in J )  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
\end{definition}
%|<<|###########################################################################################|<<|
%|<<|###########################################################################################|<<|
%|<<|###########################################################################################|<<|
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\par %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
The measurement matrix is denoted by
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Mat{\AM} \in \R^{\m \times \n}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
with the measurements, i.e., its rows, written as
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Vec{\AV}\VL{1}, \dots, \Vec{\AV}\VL{\m} \in \R^{\n}  \), such that
\(  \Mat{\AM} = ( \Vec{\AV}\VL{1} \;\cdots\; \Vec{\AV}\VL{\m} )^{\T}  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
Fixing the measurement matrix,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Mat{\AM} \in \R^{\m \times \n}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
unless specified otherwise,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \f : \R^{\n} \to \BinarySet^{\m}  \)
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
denotes an arbitrary map that satisfies
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \DistH{\f( \Vec{u} )}{\Sign( \Mat{\AM} \Vec{u} )} \leq \tauX \m  \)
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
for all \(  \Vec{u} \in \R^{\n}  \).
%
This map, \(  \f  \), can be viewed as introducing adversarial noise into the true responses,
\(  \Vec{\yV} = \Sign( \Mat{\AM} \Vec{u} ) \mapsto \f( \Vec{u} )  \).
%
Additionally, define the functions
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \h, \hf{}{} : \R^{\n} \times \R^{\n} \to \R^{\n}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
at arbitrary ordered pairs points,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  ( \Vec{u}, \Vec{v} ) \in \R^{\n} \times \R^{\n}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
by
%|>>|===========================================================================================|>>|
\begin{subequations}
\label{eqn:h:def}
\begin{gather}
  \label{eqn:h:def:h_A}
  \h( \Vec{u}, \Vec{v} )
  =
  \frac{\sqrt{2\pi}}{\m}
  \Mat{\AM}^{\T}
  \cdot \frac{1}{2}
  \bigl( \Sign( \Mat{\AM} \Vec{u} ) - \Sign( \Mat{\AM} \Vec{v} ) \bigr)
  =
  \frac{\sqrt{2\pi}}{\m}
  \sum_{\iIx=1}^{\m}
  \Vec{\AV}\VL{\iIx}
  \cdot \frac{1}{2}
  \bigl( \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{u} \rangle )
         -
         \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{v} \rangle )
  \bigr)
  ,\\ \label{eqn:h:def:h_fA}
  \hf{\Vec{u}}{\Vec{v}}
  =
  \frac{\sqrt{2\pi}}{\m}
  \Mat{\AM}^{\T}
  \cdot \frac{1}{2}
  \bigl( \f( \Vec{u} ) - \Sign( \Mat{\AM} \Vec{v} ) \bigr)
  =
  \frac{\sqrt{2\pi}}{\m}
  \sum_{\iIx=1}^{\m}
  \Vec{\AV}\VL{\iIx}
  \cdot \frac{1}{2}
  \bigl( \f( \Vec{u} )_{i}
         -
         \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{v} \rangle )
  \bigr)
,\end{gather}
\end{subequations}
%|<<|===========================================================================================|<<|
and for \(  \JX \subseteq [\n]  \), let
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \h[\JX], \hf[\JX]{}{} : \R^{\n} \times \R^{\n} \to \R^{\n}  \)
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
denote the functions given at
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  ( \Vec{u}, \Vec{v} ) \in \R^{\n} \times \R^{\n}  \)
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
by
%|>>|===========================================================================================|>>|
\begin{subequations}
\label{eqn:h_J:def}
\begin{gather}
  \label{eqn:h:def:h_AJ}
  \h[\JX]( \Vec{u}, \Vec{v} ) =
  \ThresholdSet'{\Supp( \Vec{u} ) \cup \Supp( \Vec{v} ) \cup \JX}( \h( \Vec{u}, \Vec{v} ) )
  ,\\ \label{eqn:h:def:h_fAJ}
  \hf[\JX]{\Vec{u}}{\Vec{v}} =
  \ThresholdSet'{\Supp( \Vec{u} ) \cup \Supp( \Vec{v} ) \cup \JX}( \hf{\Vec{u}}{\Vec{v}} )
.\end{gather}
\end{subequations}
%|<<|===========================================================================================|<<|
%
Note that
%|>>|===========================================================================================|>>|
\begin{gather*}
  \frac{1}{2}
  \bigl( \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{u} \rangle )
         -
         \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{v} \rangle )
  \bigr)
  =
  \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{u} \rangle )
  \cdot
  \I( \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{u} \rangle )
      \neq \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{v} \rangle ) )
%,\end{gather*}
%%|<<|===========================================================================================|<<|
%and likewise,
%%|>>|===========================================================================================|>>|
%\begin{gather*}
  \\
  \frac{1}{2}
  \bigl( \f( \Vec{u} )_{i}
         -
         \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{v} \rangle )
  \bigr)
  =
  -\Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{v} \rangle )
  \cdot
  \I( \f( \Vec{u} )_{i} \neq \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{v} \rangle ) )
.\end{gather*}
%|<<|===========================================================================================|<<|
and hence, \(  \h, \hf{}{}, \h[\JX], \hf[\JX]{}{}  \) are equivalently given by
%|>>|===========================================================================================|>>|
\begin{subequations}
\label{eqn:notation:h:def-alt}
\begin{gather}
  \label{eqn:notation:hA:def-alt}
  \h( \Vec{u}, \Vec{v} )
  =
  \frac{\sqrt{2\pi}}{\m}
  \sum_{\iIx=1}^{\m}
  \Vec{\AV}\VL{\iIx}
  \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{u} \rangle )
  \cdot
  \I( \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{u} \rangle )
      \neq \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{v} \rangle ) )
  ,\\ \label{eqn:notation:hfA:def-alt}
  \hf{\Vec{u}}{\Vec{v}}
  =
  -\frac{\sqrt{2\pi}}{\m}
  \sum_{\iIx=1}^{\m}
  \Vec{\AV}\VL{\iIx}
  \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{v} \rangle )
  \cdot \I( \f( \Vec{u} )_{i} \neq \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{v} \rangle ) )
  ,\\
  \label{eqn:notation:hAJ:def-alt}
  \h[\JX]( \Vec{u}, \Vec{v} )
  =
  \frac{\sqrt{2\pi}}{\m}
  \sum_{\iIx=1}^{\m}
  \ThresholdSet'{\Supp( \Vec{u} ) \cup \Supp( \Vec{v} ) \cup \JX}( \Vec{\AV}\VL{\iIx} )
  \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{u} \rangle )
  \cdot
  \I( \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{u} \rangle )
      \neq \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{v} \rangle ) )
  ,\\ \label{eqn:notation:hfAJ:def-alt}
  \hf[\JX]{\Vec{u}}{\Vec{v}}
  =
  -\frac{\sqrt{2\pi}}{\m}
  \sum_{\iIx=1}^{\m}
  \ThresholdSet'{\Supp( \Vec{u} ) \cup \Supp( \Vec{v} ) \cup \JX}( \Vec{\AV}\VL{\iIx} )
  \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{v} \rangle )
  \cdot \I( \f( \Vec{u} )_{i} \neq \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{v} \rangle ) )
.\end{gather}
\end{subequations}
%|<<|===========================================================================================|<<|
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\par %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
Several universal constants,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \aC, \bC, \cX{1}, \cX{2}, \cX{3}, \cX{4}, \cX{} > 0  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
appear throughout the results and analysis in this work.
%
These universal constants are fixed as follows:
%|>>|===========================================================================================|>>|
\begin{subequations}
\label{eqn:universal-constants}
\begin{align}
  &
  \aC = \aValue,
  &&
  \bC \lesssim \bCValue,
  \\
  &
  \cX{1} = \cXOneValue \in ( \cXOneValueX, \cXOneValueXX ),
  &&
  \cX{2} = \cXTwoValue \in ( \cXTwoValueX, \cXTwoValueXX ),
  \\
  &
  \cX{3} = \cXThreeValue \in ( \cXThreeValueX, \cXThreeValueXX ),
  &&
  \cX{4} = \cXFourValue \in ( \cXFourValueX, \cXFourValueXX ),
  \\
  &
  \cX{} = 4 \left( \cX{1} + \sqrt{\cX{1}^{2} + \cX{2}} \right)^{2}
        \in ( \cValue, \cValueXX ).
%  &
%  \aC = \aValue,
%  &&
%  \bC \lesssim \bCValue,
%  \\
%  &
%  \cX{1} = \cXOneValue \lesssim \cXOneValueX,
%  &&
%  \cX{2} = \cXTwoValue \lesssim \cXTwoValueX,
%  \\
%  &
%  \cX{3} = \cXThreeValue \lesssim \cXThreeValueX,
%  &&
%  \cX{4} = \cXFourValue \lesssim \cXFourValueX
%  \\
%  &
%  \cX{} = 4 \left( \cC[1] + \sqrt{\cX{1}^{2} + \cX{2} + \cX{3}} \right)^{2} \lesssim \cValue.
\end{align}
\end{subequations}
%|<<|===========================================================================================|<<|

%|>>|+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++|>>|
%|>>|+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++|>>|
%|>>|+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++|>>|
\begin{algorithm}
\label{alg:biht:normalized}
\caption{Binary iterative hard thresholding (BIHT) algorithm, normalized projections}
%
Set \( \Eta = \sqrt{2\pi} \)\;
%
%\(
%  \Vec{\tilde{x}}^{(0)}
%  =
%  \frac{\Eta}{m}
%  \MeasMat^{\T}
%  \Sgn( \MeasMat \Vec{x} )
%\)\;
%
%\(
%  \Vec{\hat{x}}^{(0)}
%  =
%  \frac
%  {\Threshold{k}( \Vec{\tilde{x}}^{(0)} )}
%  {\left\| \Threshold{k}( \Vec{\tilde{x}}^{(0)} ) \right\|_{2}}
%\)\;
%
\(
  \Vec{\hat{x}}^{(0)}
  \sim
  \SparseSphereSubspace{k}{n}
\)\;
%
\For
{\( \Iter = 1, 2, 3, \dots \)}
{
  \(
    \Vec{\tilde{x}}^{(\Iter)}
    \gets
    \Vec{\hat{x}}^{(\Iter-1)}
    +
    \frac{\eta}{m}
    \Mat{\AM}^{\T}
    \cdot
    \frac{1}{2}
    \left(
      \Sign \big( \Mat{\AM} \Vec{x} \big) - \Sign \big( \Mat{\AM} \Vec{\hat{x}}^{(\Iter-1)} \big)
    \right)
  \)\;
  \(
    \Vec{\hat{x}}^{(\Iter)}
    \gets
    \frac
    {\Threshold*{k}(\Vec{\tilde{x}}^{(\Iter)})}
    {\| \Threshold*{k}(\Vec{\tilde{x}}^{(\Iter)}) \|_{2}}
  \)\;
}
\end{algorithm}
%|<<|+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++|<<|
%|<<|+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++|<<|
%|<<|+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++|<<|

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The Restricted Approximate Invertibility Condition (\RAIC)} %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\label{section:|>prelim|>raic}                                          %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> notation-15-3-b.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Preliminaries}  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\label{section:|>prelim} %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Notations}              %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\label{section:|>prelim|>notations} %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\COMMENT{Evidently, this section needs some work..}

%Define the universal constants
%\ToDo{Fill these in.}
%%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
%%\(  \aC, \bC, \cC, \cX{1}, \cX{2}, \cX{3} > 0  \)
%%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%as
%%|>>|===========================================================================================|>>|
%\begin{subequations}
%\label{eqn:univ-consts}
%\begin{gather}
%\label{eqn:univ-consts:1}
%  \text{\ToDo{Fill these in.}}
%\end{gather}
%\end{subequations}
%%|<<|===========================================================================================|<<|

Throughout this work, the parameters \(  \k, \n \in \Z_{+}  \) are taken to satisfy
\(  \n \geq 2\k  \),
where \(  \k  \) denotes sparsity (i.e., the maximum number of nonzero entries in a vector),
and where \(  \n  \) is the dimension of the signal vectors and measurements.
%
The number of measurements (and rows in the measurement matrix) is denoted by \(  \m \in \Z_{+}  \).
%
For notational simplicity, the parameter \(  \tauX \in (0,1]  \)%
---the fraction of responses that can be corrupted---%
is assumed to satisfy
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \tauX \m \in \Z_{+}  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
This does not forgo generality since \(  \tauX \m  \) can be replaced by
\(  \lceil \tauX \m \rceil  \) throughout the analysis in this manuscript.
%
Note that this work does not consider \(  \tauX = 0  \) since \cite{matsumoto2022binary}
already established the result under noiseless conditions.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\par %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
For the purposes of this discussion, let \(  \Ell, \dX \in \Z_{+}  \),
where \(  \dX \in \Z_{+}  \) specifies an arbitrary dimension.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\par %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
Let \(  \Distr{D}  \) be an arbitrary distribution.
%
Then, \(  \RV{X} \sim \Distr{D}  \) denotes a random variable
which follows the distribution \(  \Distr{D}  \).
%
Similarly, let \(  \Set{S}  \) be an arbitrary set.
%
Then, \(  \RV{X} \sim \Set{S}  \) denotes a random variable
which follows the uniform distribution over \(  \Set{S}  \).
%
The univariate normal distribution with
mean \(  \mu \in \R  \) and variance \(  \sigma^{2} \in \R_{\geq 0}  \)
is denoted by \(  \N( \mu, \sigma^{2} )  \),
while the \(  \dX  \)-variate normal distribution with
mean vector \(  \Vec{\mu} \in \R^{\dX}  \) and
covariance matrix \(  \Mat{\Sigma} \in \R^{\dX \times \dX}  \)
is denoted by \(  \N( \Vec{\mu}, \Mat{\Sigma} )  \).
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\par %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
The \(  \dX  \)-dimensional identity matrix is denoted by \(  \Id{\dX} \in \R^{\dX \times \dX}  \).
%
More generally, matrices are written as capital letters in boldface, upright typeface, e.g.,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Mat{A} \in \R^{\Ell \times \dX}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
with the \(  i\Th  \) rows denoted by, e.g.,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Mat{A}\VL{i} \in \R^{\dX}  \), \(  i \in [\Ell]  \), such that
\(  \Mat{A} = ( \Mat{A}\VL{1} \cdots \Mat{A}\VL{\Ell} )^{\T}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
and with the \(  (i,j)  \)-entries written in italic typeface, e.g.,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Mat*{A}_{i,j} \in \R  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
Nonrandom vectors are written as lowercase letters in boldface, upright typeface, e.g.,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Vec{u} \in \R^{\dX}  \)
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
with the \(  j\Th  \) entries, \(  j \in [\dX]  \), written in italic typeface, e.g.,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Vec*{u}_{j} \in \R  \), such that
\(  \Vec{u} = ( \Vec*{u}_{1}, \dots, \Vec*{u}_{\dX} )  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
Random vectors follow the same convention as nonrandom vectors but with uppercase letters, e.g.,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Vec{Z} = ( \Vec*{Z}_{1}, \dots, \Vec*{Z}_{\dX} ) \sim \N( \Vec{0}, \Id{\dX} )  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
For \(  \JX \subseteq [\dX]  \), the restriction of \(  \Vec{u} \in \R^{\dX}  \) to the entries
indexed by \(  \JX  \) is denoted by
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Restriction{\Vec{u}}{\JX} \in \R^{| \JX |}  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
The support of a vector, \(  \Vec{u} \in \R^{\dX}  \), is denoted by
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Supp( \Vec{u} ) \defeq \{ j \in [\dX] : \Vec*{u}_{j} \neq 0 \} \subseteq [\dX]  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
and the number of nonzero entries in \(  \Vec{u}  \)%
---the \(  \lnorm{0}  \)-``norm'' of \(  \Vec{u}  \)---%
is written as
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \| \Vec{u} \|_{0} \defeq | \Supp( \Vec{u} ) |  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\par %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
The \(  \lnorm{2}  \)-unit sphere in \(  \R^{\dX}  \) is denoted by
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Sphere{\dX} \defeq \{ \Vec{u} \in \R^{\dX} : \| \Vec{u} \|_{2} = 1 \}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
and the set of \(  \k  \)-sparse \(  \dX  \)-dimensional vectors is written as
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \SparseSubspace{\k}{\dX} \defeq \{ \Vec{u} \in \R^{\dX} : \| \Vec{u} \|_{0} \leq \k \}  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
Hence, the set of all \(  \dX  \)-dimensional, \ksparserealunit vectors is denote by
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \SparseSphereSubspace{\k}{\dX} \defeq
    \{ \Vec{u} \in \Sphere{\dX} : \| \Vec{u} \|_{0} \leq \k \}  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
The distance between two points projected onto the \(  \lnorm{2}  \)-unit sphere is specified by
the function
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \DistSOp{\dX} : \R^{\dX} \times \R^{\dX} \to \R_{\geq 0}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
where
%|>>|===========================================================================================|>>|
\begin{gather*}
  \DistS[\dX]{\Vec{u}}{\Vec{v}}
  =
  \begin{cases}
  \left\| \frac{\Vec{u}}{\| \Vec{u} \|_{2}} - \frac{\Vec{v}}{\| \Vec{v} \|_{2}} \right\|_{2},
     &\cIf \Vec{u}, \Vec{v} \neq \Vec{0}, \\
  0, &\cIf \Vec{u} = \Vec{v} = \Vec{0}, \\
  1, &\cOtherwise,
  \end{cases}
\end{gather*}
%|<<|===========================================================================================|<<|
for \(  \Vec{u}, \Vec{v} \in \R^{\dX}  \).
%
The sign function, \(  \Sign. : \R \to \BinarySet  \), follows the convention:
%|>>|===========================================================================================|>>|
\begin{gather*}
  \Sign( a )
  =
  \begin{cases}
   -1, &\cIf a    < 0, \\
  \+1, &\cIf a \geq 0,
  \end{cases}
\end{gather*}
%|<<|===========================================================================================|<<|
where \(  a \in \R  \).
%
This notation extends to vectors as \(  \Sign. : \R^{\dX} \to \BinarySet^{\dX}  \)
by taking the \(  \pm  \)-signs of each entry of a \(  \dX  \)-dimensional vector.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\par %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
This work considers two notions of hard thresholding as means to project points into
the subspace of \(  \Ell  \)-sparse vectors, \(  \SparseSubspace{\Ell}{\dX}  \):
\topk[\(  \Ell  \)] and \ksubset[\(  \Ell  \)] \hardthresholding.
%
These are formalized in the following definitions.
%
%|>>|###########################################################################################|>>|
%|>>|###########################################################################################|>>|
%|>>|###########################################################################################|>>|
\begin{definition}[{\Topk[\(  \Ell  \)] \hardthresholding}]
\label{def:top-k-hard-thresholding}
%
%Let \(  \Vec{u} \in \R^{\dX}  \).
%
The \emph{\topk[\(  \Ell  \)] \hardthresholding operation}, denoted by
\(  \Threshold{\Ell} : \R^{\dX} \to \R^{\dX}  \),
projects a vector \(  \Vec{u} \in \R^{\dX}  \) into \(  \SparseSubspace{\Ell}{\dX}  \)
by retaining only the \(  \Ell  \) largest (in absolute value) entries in \(  \Vec{u}  \)
and setting all other entries to \(  0  \).
%
Note that ``ties'' can be broken arbitrarily.
%
More formally, writing
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Set{U}_{\Ell} = \{ \Vec{u'} \in \R^{\dX} : \| \Vec{u'} \|_{0} = \Ell, \ \Vec*{u'}_{j} \in \{ \Vec*{u}_{j}, 0 \} \ \forall j \in [\dX] \}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
the \topk[\(  \Ell  \)] \hardthresholding operation maps:
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(
  \Vec{u} \mapsto
  \Threshold{\Ell}( \Vec{u} )
  \in \arg\max_{\Vec{u'} \in \Set{U}_{\Ell}} \| \Vec{u'} \|_{1}
\).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
\end{definition}
%|<<|###########################################################################################|<<|
%|<<|###########################################################################################|<<|
%|<<|###########################################################################################|<<|
%
%|>>|###########################################################################################|>>|
%|>>|###########################################################################################|>>|
%|>>|###########################################################################################|>>|
\begin{definition}[{\kSubset[\(  \Ell  \)] \hardthresholding}]
\label{def:k-subset-hard-thresholding}
%
%Let
%%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
%\(  J \subseteq [\dX]  \).
%%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
The \emph{\ksubset \hardthresholding operation}
associated with a coordinate subset \(  J \subseteq [\dX]  \),
denoted by
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \ThresholdSet'{J} : \R^{\dX} \to \R^{\dX}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
takes a vector, \(  \Vec{u} \in \R^{\dX}  \), into \(  \SparseSubspace{|J|}{\dX}  \)
by setting all entries in \(  \Vec{u}  \) indexed by \(  [\dX] \setminus J  \) to \(  0  \).
%
More formally, \(  \ThresholdSet'{J}( \Vec{u} )  \) is the vector whose \(  j\Th  \) entries,
\(  j \in [\dX]  \), are given by
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \ThresholdSet*'{J}( \Vec{u} )_{j} = \Vec*{u}_{j} \cdot \I( j \in J )  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
\end{definition}
%|<<|###########################################################################################|<<|
%|<<|###########################################################################################|<<|
%|<<|###########################################################################################|<<|
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\par %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
The measurement matrix is denoted by
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Mat{\AM} \in \R^{\m \times \n}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
with the measurements, i.e., its rows, written as
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Vec{\AV}\VL{1}, \dots, \Vec{\AV}\VL{\m} \in \R^{\n}  \), such that
\(  \Mat{\AM} = ( \Vec{\AV}\VL{1} \;\cdots\; \Vec{\AV}\VL{\m} )^{\T}  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
Fixing the measurement matrix,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Mat{\AM} \in \R^{\m \times \n}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
unless specified otherwise,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \f : \R^{\n} \to \BinarySet^{\m}  \)
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
denotes an arbitrary map that satisfies
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \DistH{\f( \Vec{u} )}{\Sign( \Mat{\AM} \Vec{u} )} \leq \tauX \m  \)
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
for all \(  \Vec{u} \in \R^{\n}  \).
%
This map, \(  \f  \), can be viewed as introducing adversarial noise into the true responses,
\(  \Vec{\yV} = \Sign( \Mat{\AM} \Vec{u} ) \mapsto \f( \Vec{u} )  \).
%
At this point we can formally define the normalized BIHT algorithm. It is given as Algorithm~\ref{alg:biht:normalized} below.

\begin{algorithm}
\label{alg:biht:normalized}
\caption{Binary iterative hard thresholding (BIHT) algorithm, normalized projections}
%
Set \( \Eta = \sqrt{2\pi} \)\;
%
%\(
%  \Vec{\tilde{x}}^{(0)}
%  =
%  \frac{\Eta}{m}
%  \MeasMat^{\T}
%  \Sgn( \MeasMat \Vec{x} )
%\)\;
%
%\(
%  \Vec{\hat{x}}^{(0)}
%  =
%  \frac
%  {\Threshold{k}( \Vec{\tilde{x}}^{(0)} )}
%  {\left\| \Threshold{k}( \Vec{\tilde{x}}^{(0)} ) \right\|_{2}}
%\)\;
%
\(
  \Vec{\hat{x}}^{(0)}
  \sim
  \SparseSphereSubspace{k}{n}
\)\;
%
\For
{\( \Iter = 1, 2, 3, \dots \)}
{
  \(
    \Vec{\tilde{x}}^{(\Iter)}
    \gets
    \Vec{\hat{x}}^{(\Iter-1)}
    +
    \frac{\eta}{m}
    \Mat{\AM}^{\T}
    \cdot
    \frac{1}{2}
    \left(
      \Sign \big( \Mat{\AM} \Vec{x} \big) - \Sign \big( \Mat{\AM} \Vec{\hat{x}}^{(\Iter-1)} \big)
    \right)
  \)\;
  \(
    \Vec{\hat{x}}^{(\Iter)}
    \gets
    \frac
    {\Threshold*{k}(\Vec{\tilde{x}}^{(\Iter)})}
    {\| \Threshold*{k}(\Vec{\tilde{x}}^{(\Iter)}) \|_{2}}
  \)\;
}
\end{algorithm}


Additionally, define the functions
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \h, \hf{}{} : \R^{\n} \times \R^{\n} \to \R^{\n}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
at arbitrary ordered pairs points,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  ( \Vec{u}, \Vec{v} ) \in \R^{\n} \times \R^{\n}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
by
%|>>|===========================================================================================|>>|
\begin{subequations}
\label{eqn:h:def}
\begin{gather}
  \label{eqn:h:def:h_A}
  \h( \Vec{u}, \Vec{v} )
  =
  \frac{\sqrt{2\pi}}{\m}
  \Mat{\AM}^{\T}
  \cdot \frac{1}{2}
  \bigl( \Sign( \Mat{\AM} \Vec{u} ) - \Sign( \Mat{\AM} \Vec{v} ) \bigr)
  =
  \frac{\sqrt{2\pi}}{\m}
  \sum_{\iIx=1}^{\m}
  \Vec{\AV}\VL{\iIx}
  \cdot \frac{1}{2}
  \bigl( \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{u} \rangle )
         -
         \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{v} \rangle )
  \bigr)
  ,\\ \label{eqn:h:def:h_fA}
  \hf{\Vec{u}}{\Vec{v}}
  =
  \frac{\sqrt{2\pi}}{\m}
  \Mat{\AM}^{\T}
  \cdot \frac{1}{2}
  \bigl( \f( \Vec{u} ) - \Sign( \Mat{\AM} \Vec{v} ) \bigr)
  =
  \frac{\sqrt{2\pi}}{\m}
  \sum_{\iIx=1}^{\m}
  \Vec{\AV}\VL{\iIx}
  \cdot \frac{1}{2}
  \bigl( \f( \Vec{u} )_{i}
         -
         \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{v} \rangle )
  \bigr)
,\end{gather}
\end{subequations}
%|<<|===========================================================================================|<<|
and for \(  \JX \subseteq [\n]  \), let
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \h[\JX], \hf[\JX]{}{} : \R^{\n} \times \R^{\n} \to \R^{\n}  \)
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
denote the functions given at
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  ( \Vec{u}, \Vec{v} ) \in \R^{\n} \times \R^{\n}  \)
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
by
%|>>|===========================================================================================|>>|
\begin{subequations}
\label{eqn:h_J:def}
\begin{gather}
  \label{eqn:h:def:h_AJ}
  \h[\JX]( \Vec{u}, \Vec{v} ) =
  \ThresholdSet'{\Supp( \Vec{u} ) \cup \Supp( \Vec{v} ) \cup \JX}( \h( \Vec{u}, \Vec{v} ) )
  ,\\ \label{eqn:h:def:h_fAJ}
  \hf[\JX]{\Vec{u}}{\Vec{v}} =
  \ThresholdSet'{\Supp( \Vec{u} ) \cup \Supp( \Vec{v} ) \cup \JX}( \hf{\Vec{u}}{\Vec{v}} )
.\end{gather}
\end{subequations}
%|<<|===========================================================================================|<<|
%
Note that
%%|>>|===========================================================================================|>>|
%\begin{gather*}
%  \frac{1}{2}
%  \bigl( \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{u} \rangle )
%         -
%         \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{v} \rangle )
%  \bigr)
%  =
%  \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{u} \rangle )
%  \cdot
%  \I( \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{u} \rangle )
%      \neq \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{v} \rangle ) )
%,\end{gather*}
%%|<<|===========================================================================================|<<|
%and likewise,
%|>>|===========================================================================================|>>|
\begin{gather*}
%  \\
  \frac{1}{2}
  \bigl( \f( \Vec{u} )_{i}
         -
         \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{v} \rangle )
  \bigr)
  =
  -\Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{v} \rangle )
  \cdot
  \I( \f( \Vec{u} )_{i} \neq \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{v} \rangle ) )
.\end{gather*}
%|<<|===========================================================================================|<<|
and hence, \(  \hf{}{}, \hf[\JX]{}{}  \) are equivalently given by
%|>>|===========================================================================================|>>|
\begin{subequations}
\label{eqn:notation:h:def-alt}
\begin{gather}
%  \label{eqn:notation:hA:def-alt}
%  \h( \Vec{u}, \Vec{v} )
%  =
%  \frac{\sqrt{2\pi}}{\m}
%  \sum_{\iIx=1}^{\m}
%  \Vec{\AV}\VL{\iIx}
%  \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{u} \rangle )
%  \cdot
%  \I( \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{u} \rangle )
%      \neq \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{v} \rangle ) )
%  ,\\
  \label{eqn:notation:hfA:def-alt}
  \hf{\Vec{u}}{\Vec{v}}
  =
  -\frac{\sqrt{2\pi}}{\m}
  \sum_{\iIx=1}^{\m}
  \Vec{\AV}\VL{\iIx}
  \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{v} \rangle )
  \cdot \I( \f( \Vec{u} )_{i} \neq \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{v} \rangle ) )
%  ,\\ \label{eqn:notation:hAJ:def-alt}
%  \h[\JX]( \Vec{u}, \Vec{v} )
%  =
%  \frac{\sqrt{2\pi}}{\m}
%  \sum_{\iIx=1}^{\m}
%  \ThresholdSet'{\Supp( \Vec{u} ) \cup \Supp( \Vec{v} ) \cup \JX}( \Vec{\AV}\VL{\iIx} )
%  \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{u} \rangle )
%  \cdot
%  \I( \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{u} \rangle )
%      \neq \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{v} \rangle ) )
  ,\\ \label{eqn:notation:hfAJ:def-alt}
  \hf[\JX]{\Vec{u}}{\Vec{v}}
  =
  -\frac{\sqrt{2\pi}}{\m}
  \sum_{\iIx=1}^{\m}
  \ThresholdSet'{\Supp( \Vec{u} ) \cup \Supp( \Vec{v} ) \cup \JX}( \Vec{\AV}\VL{\iIx} )
  \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{v} \rangle )
  \cdot \I( \f( \Vec{u} )_{i} \neq \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{v} \rangle ) )
.\end{gather}
\end{subequations}
%|<<|===========================================================================================|<<|
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\par %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
Several universal constants,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \aC, \bC, \cX{1}, \cX{2}, \cX{3}, \cX{4}, \cX{} > 0  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
appear throughout the results and analysis in this work.
%
These universal constants are fixed as follows:
%|>>|===========================================================================================|>>|
\begin{subequations}
\label{eqn:universal-constants}
\begin{align}
  &
  \aC = \aValue,
  &&
  \bC \lesssim \bCValue,
  \\
  &
  \cX{1} = \cXOneValue \in ( \cXOneValueX, \cXOneValueXX ),
  &&
  \cX{2} = \cXTwoValue \in ( \cXTwoValueX, \cXTwoValueXX ),
  \\
  &
  \cX{3} = \cXThreeValue \in ( \cXThreeValueX, \cXThreeValueXX ),
  &&
  \cX{4} = \cXFourValue \in ( \cXFourValueX, \cXFourValueXX ),
  \\
  &
  \cX{} = 4 \left( \cX{1} + \sqrt{\cX{1}^{2} + \cX{2}} \right)^{2}
        \in ( \cValue, \cValueXX ).
%  &
%  \aC = \aValue,
%  &&
%  \bC \lesssim \bCValue,
%  \\
%  &
%  \cX{1} = \cXOneValue \lesssim \cXOneValueX,
%  &&
%  \cX{2} = \cXTwoValue \lesssim \cXTwoValueX,
%  \\
%  &
%  \cX{3} = \cXThreeValue \lesssim \cXThreeValueX,
%  &&
%  \cX{4} = \cXFourValue \lesssim \cXFourValueX
%  \\
%  &
%  \cX{} = 4 \left( \cC[1] + \sqrt{\cX{1}^{2} + \cX{2} + \cX{3}} \right)^{2} \lesssim \cValue.
\end{align}
\end{subequations}
%|<<|===========================================================================================|<<|

%|>>|+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++|>>|
%|>>|+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++|>>|
%|>>|+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++|>>|

%|<<|+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++|<<|
%|<<|+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++|<<|
%|<<|+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++|<<|

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The Restricted Approximate Invertibility Condition (\RAIC)} %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\label{section:|>prelim|>raic}                                          %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> notation-15-3.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Preliminaries}  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\label{section:|>prelim} %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Notations}              %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\label{section:|>prelim|>notations} %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\COMMENT{Evidently, this section needs some work..}

%Define the universal constants
%\ToDo{Fill these in.}
%%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
%%\(  \aC, \bC, \cC, \cX{1}, \cX{2}, \cX{3} > 0  \)
%%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%as
%%|>>|===========================================================================================|>>|
%\begin{subequations}
%\label{eqn:univ-consts}
%\begin{gather}
%\label{eqn:univ-consts:1}
%  \text{\ToDo{Fill these in.}}
%\end{gather}
%\end{subequations}
%%|<<|===========================================================================================|<<|

Throughout this work, the parameters \(  \k, \n \in \Z_{+}  \) are taken to satisfy
\(  \n \geq 2\k  \),
where \(  \k  \) denotes sparsity (i.e., the maximum number of nonzero entries in a vector),
and where \(  \n  \) is the dimension of the signal vectors and measurements.
%
The number of measurements (and rows in the measurement matrix) is denoted by \(  \m \in \Z_{+}  \).
%
For notational simplicity, the parameter \(  \tauX \in (0,1]  \)%
---the fraction of responses that can be corrupted---%
is assumed to satisfy
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \tauX \m \in \Z_{+}  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
This does not forgo generality since \(  \tauX \m  \) can be replaced by
\(  \lceil \tauX \m \rceil  \) throughout the analysis in this manuscript.
%
Note that this work does not consider \(  \tauX = 0  \) since \cite{matsumoto2022binary}
already established the result under noiseless conditions.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\par %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
For the purposes of this discussion, let \(  \Ell, \dX \in \Z_{+}  \),
where \(  \dX \in \Z_{+}  \) specifies an arbitrary dimension.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\par %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
Let \(  \Distr{D}  \) be an arbitrary distribution.
%
Then, \(  \RV{X} \sim \Distr{D}  \) denotes a random variable
which follows the distribution \(  \Distr{D}  \).
%
Similarly, let \(  \Set{S}  \) be an arbitrary set.
%
Then, \(  \RV{X} \sim \Set{S}  \) denotes a random variable
which follows the uniform distribution over \(  \Set{S}  \).
%
The univariate normal distribution with
mean \(  \mu \in \R  \) and variance \(  \sigma^{2} \in \R_{\geq 0}  \)
is denoted by \(  \N( \mu, \sigma^{2} )  \),
while the \(  \dX  \)-variate normal distribution with
mean vector \(  \Vec{\mu} \in \R^{\dX}  \) and
covariance matrix \(  \Mat{\Sigma} \in \R^{\dX \times \dX}  \)
is denoted by \(  \N( \Vec{\mu}, \Mat{\Sigma} )  \).
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\par %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
The \(  \dX  \)-dimensional identity matrix is denoted by \(  \Id{\dX} \in \R^{\dX \times \dX}  \).
%
More generally, matrices are written as capital letters in boldface, upright typeface, e.g.,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Mat{A} \in \R^{\Ell \times \dX}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
with the \(  i\Th  \) rows denoted by, e.g.,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Mat{A}\VL{i} \in \R^{\dX}  \), \(  i \in [\Ell]  \), such that
\(  \Mat{A} = ( \Mat{A}\VL{1} \cdots \Mat{A}\VL{\Ell} )^{\T}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
and with the \(  (i,j)  \)-entries written in italic typeface, e.g.,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Mat*{A}_{i,j} \in \R  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
Nonrandom vectors are written as lowercase letters in boldface, upright typeface, e.g.,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Vec{u} \in \R^{\dX}  \)
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
with the \(  j\Th  \) entries, \(  j \in [\dX]  \), written in italic typeface, e.g.,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Vec*{u}_{j} \in \R  \), such that
\(  \Vec{u} = ( \Vec*{u}_{1}, \dots, \Vec*{u}_{\dX} )  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
Random vectors follow the same convention as nonrandom vectors but with uppercase letters, e.g.,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Vec{Z} = ( \Vec*{Z}_{1}, \dots, \Vec*{Z}_{\dX} ) \sim \N( \Vec{0}, \Id{\dX} )  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
For \(  \JX \subseteq [\dX]  \), the restriction of \(  \Vec{u} \in \R^{\dX}  \) to the entries
indexed by \(  \JX  \) is denoted by
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Restriction{\Vec{u}}{\JX} \in \R^{| \JX |}  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
The support of a vector, \(  \Vec{u} \in \R^{\dX}  \), is denoted by
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Supp( \Vec{u} ) \defeq \{ j \in [\dX] : \Vec*{u}_{j} \neq 0 \} \subseteq [\dX]  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
and the number of nonzero entries in \(  \Vec{u}  \)%
---the \(  \lnorm{0}  \)-``norm'' of \(  \Vec{u}  \)---%
is written as
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \| \Vec{u} \|_{0} \defeq | \Supp( \Vec{u} ) |  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\par %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
The \(  \lnorm{2}  \)-unit sphere in \(  \R^{\dX}  \) is denoted by
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Sphere{\dX} \defeq \{ \Vec{u} \in \R^{\dX} : \| \Vec{u} \|_{2} = 1 \}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
and the set of \(  \k  \)-sparse \(  \dX  \)-dimensional vectors is written as
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \SparseSubspace{\k}{\dX} \defeq \{ \Vec{u} \in \R^{\dX} : \| \Vec{u} \|_{0} \leq \k \}  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
Hence, the set of all \(  \dX  \)-dimensional, \ksparserealunit vectors is denote by
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \SparseSphereSubspace{\k}{\dX} \defeq
    \{ \Vec{u} \in \Sphere{\dX} : \| \Vec{u} \|_{0} \leq \k \}  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
The distance between two points projected onto the \(  \lnorm{2}  \)-unit sphere is specified by
the function
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \DistSOp{\dX} : \R^{\dX} \times \R^{\dX} \to \R_{\geq 0}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
where
%|>>|===========================================================================================|>>|
\begin{gather*}
  \DistS[\dX]{\Vec{u}}{\Vec{v}}
  =
  \begin{cases}
  \left\| \frac{\Vec{u}}{\| \Vec{u} \|_{2}} - \frac{\Vec{v}}{\| \Vec{v} \|_{2}} \right\|_{2},
     &\cIf \Vec{u}, \Vec{v} \neq \Vec{0}, \\
  0, &\cIf \Vec{u} = \Vec{v} = \Vec{0}, \\
  1, &\cOtherwise,
  \end{cases}
\end{gather*}
%|<<|===========================================================================================|<<|
for \(  \Vec{u}, \Vec{v} \in \R^{\dX}  \).
%
The sign function, \(  \Sign. : \R \to \BinarySet  \), follows the convention:
%|>>|===========================================================================================|>>|
\begin{gather*}
  \Sign( a )
  =
  \begin{cases}
   -1, &\cIf a    < 0, \\
  \+1, &\cIf a \geq 0,
  \end{cases}
\end{gather*}
%|<<|===========================================================================================|<<|
where \(  a \in \R  \).
%
This notation extends to vectors as \(  \Sign. : \R^{\dX} \to \BinarySet^{\dX}  \)
by taking the \(  \pm  \)-signs of each entry of a \(  \dX  \)-dimensional vector.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\par %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
This work considers two notions of hard thresholding as means to project points into
the subspace of \(  \Ell  \)-sparse vectors, \(  \SparseSubspace{\Ell}{\dX}  \):
\topk[\(  \Ell  \)] and \ksubset[\(  \Ell  \)] \hardthresholding.
%
These are formalized in the following definitions.
%
%|>>|###########################################################################################|>>|
%|>>|###########################################################################################|>>|
%|>>|###########################################################################################|>>|
\begin{definition}[{\Topk[\(  \Ell  \)] \hardthresholding}]
\label{def:top-k-hard-thresholding}
%
%Let \(  \Vec{u} \in \R^{\dX}  \).
%
The \emph{\topk[\(  \Ell  \)] \hardthresholding operation}, denoted by
\(  \Threshold{\Ell} : \R^{\dX} \to \R^{\dX}  \),
projects a vector \(  \Vec{u} \in \R^{\dX}  \) into \(  \SparseSubspace{\Ell}{\dX}  \)
by retaining only the \(  \Ell  \) largest (in absolute value) entries in \(  \Vec{u}  \)
and setting all other entries to \(  0  \).
%
Note that ``ties'' can be broken arbitrarily.
%
More formally, writing
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Set{U}_{\Ell} = \{ \Vec{u'} \in \R^{\dX} : \| \Vec{u'} \|_{0} = \Ell, \ \Vec*{u'}_{j} \in \{ \Vec*{u}_{j}, 0 \} \ \forall j \in [\dX] \}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
the \topk[\(  \Ell  \)] \hardthresholding operation maps:
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(
  \Vec{u} \mapsto
  \Threshold{\Ell}( \Vec{u} )
  \in \arg\max_{\Vec{u'} \in \Set{U}_{\Ell}} \| \Vec{u'} \|_{1}
\).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
\end{definition}
%|<<|###########################################################################################|<<|
%|<<|###########################################################################################|<<|
%|<<|###########################################################################################|<<|
%
%|>>|###########################################################################################|>>|
%|>>|###########################################################################################|>>|
%|>>|###########################################################################################|>>|
\begin{definition}[{\kSubset[\(  \Ell  \)] \hardthresholding}]
\label{def:k-subset-hard-thresholding}
%
%Let
%%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
%\(  J \subseteq [\dX]  \).
%%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
The \emph{\ksubset \hardthresholding operation}
associated with a coordinate subset \(  J \subseteq [\dX]  \),
denoted by
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \ThresholdSet'{J} : \R^{\dX} \to \R^{\dX}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
takes a vector, \(  \Vec{u} \in \R^{\dX}  \), into \(  \SparseSubspace{|J|}{\dX}  \)
by setting all entries in \(  \Vec{u}  \) indexed by \(  [\dX] \setminus J  \) to \(  0  \).
%
More formally, \(  \ThresholdSet'{J}( \Vec{u} )  \) is the vector whose \(  j\Th  \) entries,
\(  j \in [\dX]  \), are given by
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \ThresholdSet*'{J}( \Vec{u} )_{j} = \Vec*{u}_{j} \cdot \I( j \in J )  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
\end{definition}
%|<<|###########################################################################################|<<|
%|<<|###########################################################################################|<<|
%|<<|###########################################################################################|<<|
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\par %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
The measurement matrix is denoted by
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Mat{\AM} \in \R^{\m \times \n}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
with the measurements, i.e., its rows, written as
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Vec{\AV}\VL{1}, \dots, \Vec{\AV}\VL{\m} \in \R^{\n}  \), such that
\(  \Mat{\AM} = ( \Vec{\AV}\VL{1} \;\cdots\; \Vec{\AV}\VL{\m} )^{\T}  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
Fixing the measurement matrix,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Mat{\AM} \in \R^{\m \times \n}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
unless specified otherwise,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \f : \R^{\n} \to \BinarySet^{\m}  \)
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
denotes an arbitrary map that satisfies
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \DistH{\f( \Vec{u} )}{\Sign( \Mat{\AM} \Vec{u} )} \leq \tauX \m  \)
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
for all \(  \Vec{u} \in \R^{\n}  \).
%
This map, \(  \f  \), can be viewed as introducing adversarial noise into the true responses,
\(  \Vec{\yV} = \Sign( \Mat{\AM} \Vec{u} ) \mapsto \f( \Vec{u} )  \).
%
At this point we can formally define the normalized BIHT algorithm. It is given as Algorithm~\ref{alg:biht:normalized} below.

\begin{algorithm}
\label{alg:biht:normalized}
\caption{Binary iterative hard thresholding (BIHT) algorithm, normalized projections}
%
Set \( \Eta = \sqrt{2\pi} \)\;
%
%\(
%  \Vec{\tilde{x}}^{(0)}
%  =
%  \frac{\Eta}{m}
%  \MeasMat^{\T}
%  \Sgn( \MeasMat \Vec{x} )
%\)\;
%
%\(
%  \Vec{\hat{x}}^{(0)}
%  =
%  \frac
%  {\Threshold{k}( \Vec{\tilde{x}}^{(0)} )}
%  {\left\| \Threshold{k}( \Vec{\tilde{x}}^{(0)} ) \right\|_{2}}
%\)\;
%
\(
  \Vec{\hat{x}}^{(0)}
  \sim
  \SparseSphereSubspace{k}{n}
\)\;
%
\For
{\( \Iter = 1, 2, 3, \dots \)}
{
  \(
    \Vec{\tilde{x}}^{(\Iter)}
    \gets
    \Vec{\hat{x}}^{(\Iter-1)}
    +
    \frac{\eta}{m}
    \Mat{\AM}^{\T}
    \cdot
    \frac{1}{2}
    \left(
      \Sign \big( \Mat{\AM} \Vec{x} \big) - \Sign \big( \Mat{\AM} \Vec{\hat{x}}^{(\Iter-1)} \big)
    \right)
  \)\;
  \(
    \Vec{\hat{x}}^{(\Iter)}
    \gets
    \frac
    {\Threshold*{k}(\Vec{\tilde{x}}^{(\Iter)})}
    {\| \Threshold*{k}(\Vec{\tilde{x}}^{(\Iter)}) \|_{2}}
  \)\;
}
\end{algorithm}


Additionally, define the functions
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \h, \hf{}{} : \R^{\n} \times \R^{\n} \to \R^{\n}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
at arbitrary ordered pairs points,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  ( \Vec{u}, \Vec{v} ) \in \R^{\n} \times \R^{\n}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
by
%|>>|===========================================================================================|>>|
\begin{subequations}
\label{eqn:h:def}
\begin{gather}
  \label{eqn:h:def:h_A}
  \h( \Vec{u}, \Vec{v} )
  =
  \frac{\sqrt{2\pi}}{\m}
  \Mat{\AM}^{\T}
  \cdot \frac{1}{2}
  \bigl( \Sign( \Mat{\AM} \Vec{u} ) - \Sign( \Mat{\AM} \Vec{v} ) \bigr)
  =
  \frac{\sqrt{2\pi}}{\m}
  \sum_{\iIx=1}^{\m}
  \Vec{\AV}\VL{\iIx}
  \cdot \frac{1}{2}
  \bigl( \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{u} \rangle )
         -
         \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{v} \rangle )
  \bigr)
  ,\\ \label{eqn:h:def:h_fA}
  \hf{\Vec{u}}{\Vec{v}}
  =
  \frac{\sqrt{2\pi}}{\m}
  \Mat{\AM}^{\T}
  \cdot \frac{1}{2}
  \bigl( \f( \Vec{u} ) - \Sign( \Mat{\AM} \Vec{v} ) \bigr)
  =
  \frac{\sqrt{2\pi}}{\m}
  \sum_{\iIx=1}^{\m}
  \Vec{\AV}\VL{\iIx}
  \cdot \frac{1}{2}
  \bigl( \f( \Vec{u} )_{i}
         -
         \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{v} \rangle )
  \bigr)
,\end{gather}
\end{subequations}
%|<<|===========================================================================================|<<|
and for \(  \JX \subseteq [\n]  \), let
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \h[\JX], \hf[\JX]{}{} : \R^{\n} \times \R^{\n} \to \R^{\n}  \)
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
denote the functions given at
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  ( \Vec{u}, \Vec{v} ) \in \R^{\n} \times \R^{\n}  \)
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
by
%|>>|===========================================================================================|>>|
\begin{subequations}
\label{eqn:h_J:def}
\begin{gather}
  \label{eqn:h:def:h_AJ}
  \h[\JX]( \Vec{u}, \Vec{v} ) =
  \ThresholdSet'{\Supp( \Vec{u} ) \cup \Supp( \Vec{v} ) \cup \JX}( \h( \Vec{u}, \Vec{v} ) )
  ,\\ \label{eqn:h:def:h_fAJ}
  \hf[\JX]{\Vec{u}}{\Vec{v}} =
  \ThresholdSet'{\Supp( \Vec{u} ) \cup \Supp( \Vec{v} ) \cup \JX}( \hf{\Vec{u}}{\Vec{v}} )
.\end{gather}
\end{subequations}
%|<<|===========================================================================================|<<|
%
Note that
%|>>|===========================================================================================|>>|
\begin{gather*}
  \frac{1}{2}
  \bigl( \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{u} \rangle )
         -
         \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{v} \rangle )
  \bigr)
  =
  \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{u} \rangle )
  \cdot
  \I( \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{u} \rangle )
      \neq \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{v} \rangle ) )
%,\end{gather*}
%%|<<|===========================================================================================|<<|
%and likewise,
%%|>>|===========================================================================================|>>|
%\begin{gather*}
  \\
  \frac{1}{2}
  \bigl( \f( \Vec{u} )_{i}
         -
         \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{v} \rangle )
  \bigr)
  =
  -\Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{v} \rangle )
  \cdot
  \I( \f( \Vec{u} )_{i} \neq \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{v} \rangle ) )
.\end{gather*}
%|<<|===========================================================================================|<<|
and hence, \(  \h, \hf{}{}, \h[\JX], \hf[\JX]{}{}  \) are equivalently given by
%|>>|===========================================================================================|>>|
\begin{subequations}
\label{eqn:notation:h:def-alt}
\begin{gather}
  \label{eqn:notation:hA:def-alt}
  \h( \Vec{u}, \Vec{v} )
  =
  \frac{\sqrt{2\pi}}{\m}
  \sum_{\iIx=1}^{\m}
  \Vec{\AV}\VL{\iIx}
  \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{u} \rangle )
  \cdot
  \I( \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{u} \rangle )
      \neq \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{v} \rangle ) )
  ,\\ \label{eqn:notation:hfA:def-alt}
  \hf{\Vec{u}}{\Vec{v}}
  =
  -\frac{\sqrt{2\pi}}{\m}
  \sum_{\iIx=1}^{\m}
  \Vec{\AV}\VL{\iIx}
  \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{v} \rangle )
  \cdot \I( \f( \Vec{u} )_{i} \neq \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{v} \rangle ) )
  ,\\
  \label{eqn:notation:hAJ:def-alt}
  \h[\JX]( \Vec{u}, \Vec{v} )
  =
  \frac{\sqrt{2\pi}}{\m}
  \sum_{\iIx=1}^{\m}
  \ThresholdSet'{\Supp( \Vec{u} ) \cup \Supp( \Vec{v} ) \cup \JX}( \Vec{\AV}\VL{\iIx} )
  \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{u} \rangle )
  \cdot
  \I( \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{u} \rangle )
      \neq \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{v} \rangle ) )
  ,\\ \label{eqn:notation:hfAJ:def-alt}
  \hf[\JX]{\Vec{u}}{\Vec{v}}
  =
  -\frac{\sqrt{2\pi}}{\m}
  \sum_{\iIx=1}^{\m}
  \ThresholdSet'{\Supp( \Vec{u} ) \cup \Supp( \Vec{v} ) \cup \JX}( \Vec{\AV}\VL{\iIx} )
  \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{v} \rangle )
  \cdot \I( \f( \Vec{u} )_{i} \neq \Sign( \langle \Vec{\AV}\VL{\iIx}, \Vec{v} \rangle ) )
.\end{gather}
\end{subequations}
%|<<|===========================================================================================|<<|
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\par %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
Several universal constants,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \aC, \bC, \cX{1}, \cX{2}, \cX{3}, \cX{4}, \cX{} > 0  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
appear throughout the results and analysis in this work.
%
These universal constants are fixed as follows:
%|>>|===========================================================================================|>>|
\begin{subequations}
\label{eqn:universal-constants}
\begin{align}
  &
  \aC = \aValue,
  &&
  \bC \lesssim \bCValue,
  \\
  &
  \cX{1} = \cXOneValue \in ( \cXOneValueX, \cXOneValueXX ),
  &&
  \cX{2} = \cXTwoValue \in ( \cXTwoValueX, \cXTwoValueXX ),
  \\
  &
  \cX{3} = \cXThreeValue \in ( \cXThreeValueX, \cXThreeValueXX ),
  &&
  \cX{4} = \cXFourValue \in ( \cXFourValueX, \cXFourValueXX ),
  \\
  &
  \cX{} = 4 \left( \cX{1} + \sqrt{\cX{1}^{2} + \cX{2}} \right)^{2}
        \in ( \cValue, \cValueXX ).
%  &
%  \aC = \aValue,
%  &&
%  \bC \lesssim \bCValue,
%  \\
%  &
%  \cX{1} = \cXOneValue \lesssim \cXOneValueX,
%  &&
%  \cX{2} = \cXTwoValue \lesssim \cXTwoValueX,
%  \\
%  &
%  \cX{3} = \cXThreeValue \lesssim \cXThreeValueX,
%  &&
%  \cX{4} = \cXFourValue \lesssim \cXFourValueX
%  \\
%  &
%  \cX{} = 4 \left( \cC[1] + \sqrt{\cX{1}^{2} + \cX{2} + \cX{3}} \right)^{2} \lesssim \cValue.
\end{align}
\end{subequations}
%|<<|===========================================================================================|<<|

%|>>|+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++|>>|
%|>>|+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++|>>|
%|>>|+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++|>>|

%|<<|+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++|<<|
%|<<|+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++|<<|
%|<<|+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++|<<|

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The Restricted Approximate Invertibility Condition (\RAIC)} %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\label{section:|>prelim|>raic}                                          %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> overview-15-2-a.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Technical Overview}         %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\label{section:|>technical-overview} %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\COMMENT{Needs some work..}

The proof of the main theorem, \THEOREM \ref{thm:adversarial},
is broadly divided into three steps, each considered under (bounded) adversarial noise:
\Enum[\label{enum:stochastic}]{\thesection.I} establish a stochastic result for Gaussian measurements,
\Enum[\label{enum:deterministic}]{\thesection.II} establish a deterministic result for the iterative approximation errors of \BIHT with arbitrary measurements, and
\Enum[\label{enum:combine}]{\thesection.III} combine \ref{enum:stochastic} and \ref{enum:deterministic} to characterize the convergence of \BIHT under adversarial noise.
%
The result obtained in \STEP \ref{enum:stochastic} establishes
the \RAIC for Gaussian measurements under adversarial noise
(\see \THEOREM \ref{thm:raic:adv}) by upper bounding:
%|>>|===========================================================================================|>>|
\begin{gather}
\label{eqn:enum:stochastic}
  \bigl\| ( \Vec{\xV} - \Vec{\yV} ) - \hf[\JX]{\Vec{\xV}}{\Vec{\yV}} \bigr\|_{2}
  \leq
  \BigO'(
    \sqrt{\epsilonRAICadv \DistS{\Vec{x}}{\Vec{y}}}
    +
    \epsilonRAICadv
    +
    \tauX %\Log( \Tfrac{1}{\tauX} )
  )
\end{gather}
%|<<|===========================================================================================|<<|
uniformly with high probability
for all \(  \Vec{\xV}, \Vec{\yV} \in \SparseSphereSubspace{\k}{\n}  \).
%
The result derived in \STEP \ref{enum:deterministic} upper bounds
the error of the \(  \Iter\Th  \) \BIHT approximations deterministically
by an expression similar to that in the definition of the \RAIC
(\see \LEMMA \ref{lemma:error:deterministic}):
%|>>|===========================================================================================|>>|
\begin{gather}
\label{eqn:enum:deterministic}
  \DistS{\Vec{\x}}{\Vec{\xApprox}\IL{\Iter}}
  \leq
  \BigO(
    \bigl\| ( \Vec{\x} - \Vec{\xApprox}\IL{\Iter-1} ) - \hf[\JX]{\Vec{\x}}{\Vec{\xApprox}\IL{\Iter-1}} \bigr\|_{2}
  )
.\end{gather}
%|<<|===========================================================================================|<<|
%
Lastly, for \STEP \ref{enum:combine}, upon the establishment of
\EQUATIONS \eqref{eqn:enum:stochastic} and \eqref{eqn:enum:deterministic},
the two equations taken together will bound the \(  \Iter\Th  \) approximation errors by:
%|>>|===========================================================================================|>>|
\begin{gather}
\label{eqn:enum:combine}
  \DistS{\Vec{\x}}{\Vec{\xApprox}\IL{\Iter}}
  \leq
  \begin{cases}
  2, &\cIf \Iter = 0, \\
  \BigO*'(
    \sqrt{\epsilonRAICadv \DistS{\Vec{\x}}{\Vec{\xApprox}\IL{\Iter-1}}}
    +
    \epsilonRAICadv
    +
    \tauX %\Log( \Tfrac{1}{\tauX} )
  ),
  &\cIf \Iter > 0.
  \end{cases}
\end{gather}
%|<<|===========================================================================================|<<|
%
Note, however, that the above expression states the upper bound on the approximation error
as a recurrence relation, rather than a closed-form result.
%
Hence, \STEP \ref{enum:combine} will also derive a closed-form expression for
\EQUATION \eqref{eqn:enum:combine} (\see \LEMMA \ref{lemma:error:recurrence}),
where much of the technical work here
has already been accomplished by \cite{matsumoto2022binary}.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\par %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
The majority of the analysis focuses on the stochastic result in \STEP \ref{enum:stochastic},
which is the main technical contribution of this work,
while the analyses for the deterministic bound in \STEP \ref{enum:deterministic}
and the final step, \STEP \ref{enum:combine},
are less involved but allow the \RAIC established in \STEP \ref{enum:stochastic}
to be related to the error of the approximations produced by the \BIHT algorithm
with corrupted responses.
%
The arguments for \STEP \ref{enum:stochastic} are briefly outlined below.
%which culminate into the proof of \THEOREM \ref{thm:raic:adv}, the main technical theorem.
%
On the other hand, \STEPS \ref{enum:deterministic} and \ref{enum:combine}
are less technically demanding and hence omitted from this overview
(\see \LEMMAS \ref{lemma:error:deterministic} and \ref{lemma:error:recurrence} and their proofs).
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Overview of the Argument for \STEP \ref{enum:stochastic}.} %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
The idea behind the approach to \THEOREM \ref{thm:raic:adv} is the following.
%
There is a (roughly) linear relationship between the expected norm of the sum of up to \(  \tauX \m  \)-many measurements and the expected error from adversarially corrupting up to \(  \tauX \m  \)-many responses. Hence, since the norm of the sum of every choice of up to \(  \tauX \m  \)-many measurements can be uniformly bounded as not ``too large'' with high probability, the error induced by the adversarial noise is similarly upper bounded with high probability.

%The two-sentence idea for the approach to the proof of \THEOREM \ref{thm:raic:adv} is:
%\emph{there is a (roughly) linear relationship between the norm of the sum of up to \(  \tauX \m  \) measurements and (an upper bound on) the amount of error that an adversary imposes by choosing to corrupt the corresponding responses. However, with high probability, the norm of every sum of at most \(  \tauX \m  \) measurements (or their negations)---and hence, also the error due to the adversarial noise---is not ``too large.''}
%\emph{what is the probability that there exists a subset of at most \(  \tauX \m  \) measurements (or their negations) whose sum has a large norm---where this quantity is related to the amount of error that an adversary imposes by choosing to corrupt these up to \(  \tauX \m  \) corresponding responses?}
%
More precisely, the argument for \THEOREM \ref{thm:raic:adv} is broken down into a few steps:
%|>>|XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXX|>>|
\Enum[\label{enum:step:A:a}]{a}~%
First, applying the triangle inequality, it can be shown that
%|>>|===========================================================================================|>>|
\begin{gather}
\label{eqn:enum:step:A:a}
  \bigl\| ( \Vec{\xV} - \Vec{\yV} ) - \hf[\JX]{\Vec{\xV}}{\Vec{\yV}} \bigr\|_{2}
  \leq
  \bigl\| ( \Vec{\xV} - \Vec{\yV} ) - \h[\JX]( \Vec{\xV}, \Vec{\yV} ) \bigr\|_{2}
  +
  \bigl\| \hf[\JX]{\Vec{\xV}}{\Vec{\xV}} \bigr\|_{2}
.\end{gather}
%|<<|===========================================================================================|<<|
%
Then, the focus of the subsequent two steps is upper bounding
the two terms on the \RHS of the above inequality.
%
Note that \EQUATION \eqref{eqn:enum:step:A:a} gives a roughly linear dependence
of the approximation error on the amount of adversarial noise.
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
\Enum[\label{enum:step:A:b}]{b}~%
The first term on the \RHS of \EQUATION \eqref{eqn:enum:step:A:a} can be upper bounded
by directly applying \cite[\THEOREM 3.3]{matsumoto2022binary}.
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
\Enum[\label{enum:step:A:c}]{c}~%
On the other hand, the rightmost term in \EQUATION \eqref{eqn:enum:step:A:a}---%
which (roughly) quantifies the amount of error caused by adversarial noise---%
requires new analysis.
%
As the first step towards bounding this term, it will be argued that it suffices to
bound each element in the image of \(  \hf[\JX]{}{}  \), where
\(  \hf[\JX]{}{} [ \PREIMG ]  \) has a finite and easily quantifiable size.
%
Note that this approach will lead to a uniform bound on
the norm of the image of \(  \hf[\JX]{}{}  \) at every real-valued point,
\(  ( \Vec{\xV}, \Vec{\xV} )  \), \(  \Vec{\xV} \in \R^{\n}  \).
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
\Enum[\label{enum:step:A:d}]{d}~%
Finally, such a uniform bound is obtained by bounding the norm of
the image of \(  \hf[\JX]{}{}  \) at an arbitrary point \(  ( \Vec{\uV}, \Vec{\uV} )  \),
and subsequently union bounding over a specifically constructed set of such points.
%
This step will orthogonally decompose \(  \hf[\JX]{\Vec{\uV}}{\Vec{\uV}}  \) into two components,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \langle \Vec{\uV}, \hf[\JX]{\Vec{\uV}}{\Vec{\uV}} \rangle \Vec{\uV}  \) and
\(  \hf[\JX]{\Vec{\uV}}{\Vec{\uV}} - \langle \Vec{\uV}, \hf[\JX]{\Vec{\uV}}{\Vec{\uV}} \rangle \Vec{\uV}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
such that
%|>>|===========================================================================================|>>|
\begin{gather*}
  \hf[\JX]{\Vec{\uV}}{\Vec{\uV}}
  =
  \langle \Vec{\uV}, \hf[\JX]{\Vec{\uV}}{\Vec{\uV}} \rangle \Vec{\uV}
  +
  \Bigl( \hf[\JX]{\Vec{\uV}}{\Vec{\uV}}
         - \langle \Vec{\uV}, \hf[\JX]{\Vec{\uV}}{\Vec{\uV}} \rangle \Vec{\uV} \Bigr)
.\end{gather*}
%|<<|===========================================================================================|<<|
%
The norm of each of the two components will be individually upper bounded
using concentration inequalities for functions of Gaussians,
and subsequently, these bounds will be combined via the triangle inequality,
%|>>|===========================================================================================|>>|
\begin{gather}
  \left\| \hf[\JX]{\Vec{\uV}}{\Vec{\uV}} \right\|_{2}
  \leq
  \left| \langle \Vec{\uV}, \hf[\JX]{\Vec{\uV}}{\Vec{\uV}} \rangle \right|
  +
  \left\| \hf[\JX]{\Vec{\uV}}{\Vec{\uV}}
          - \langle \Vec{\uV}, \hf[\JX]{\Vec{\uV}}{\Vec{\uV}} \rangle \Vec{\uV} \right\|_{2}
,\end{gather}
%|<<|===========================================================================================|<<|
and a union bound.
%|<<|XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXX|<<|

==> pf-raic-adv-1--1.tex <==
%|>>|~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~|>>|
%|>>|~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~|>>|
%|>>|~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~|>>|
\begin{proof}
{\CLAIM \ref{claim:raic:adv:3}}
%
The claim directly follows from the orthogonal decomposition discussed above
and the triangle inequality:
%|>>|===========================================================================================|>>|
\begin{align*}
  \DXXu
  &=
  \left\| \hZf[\JX]{\Vec{\uV}}{\Vec{\uV}} \right\|_{2}
  \\
  &\dCmt{by the definition of the random variable \(  \DXXu  \)}
  \\
  &=
  \left\|
    \langle \Vec{\uV}, \hZf[\JX]{\Vec{\uV}}{\Vec{\uV}} \rangle \Vec{\uV}
    +
    \bigl( \hZf[\JX]{\Vec{\uV}}{\Vec{\uV}}
           - \langle \Vec{\uV}, \hZf[\JX]{\Vec{\uV}}{\Vec{\uV}} \rangle \Vec{\uV} \bigr)
  \right\|_{2}
  \\
  &\dCmt{by \EQUATION \eqref{eqn:raic:adv:1}}
  \\
  &\leq
  \left\|
    \langle \Vec{\uV}, \hZf[\JX]{\Vec{\uV}}{\Vec{\uV}} \rangle \Vec{\uV}
  \right\|_{2}
  +
  \left\|
    \hZf[\JX]{\Vec{\uV}}{\Vec{\uV}}
    - \langle \Vec{\uV}, \hZf[\JX]{\Vec{\uV}}{\Vec{\uV}} \rangle \Vec{\uV}
  \right\|_{2}
  \\
  &\dCmt{by the triangle inequality}
  \\
  &\leq
  \left|
    \langle \Vec{\uV}, \hZf[\JX]{\Vec{\uV}}{\Vec{\uV}} \rangle
  \right|
  \| \Vec{\uV} \|_{2}
  +
  \left\|
    \hZf[\JX]{\Vec{\uV}}{\Vec{\uV}}
    - \langle \Vec{\uV}, \hZf[\JX]{\Vec{\uV}}{\Vec{\uV}} \rangle \Vec{\uV}
  \right\|_{2}
  \\
  &\dCmt{due to the homogeneity of norms}
  \\
  &\leq
  \left|
    \langle \Vec{\uV}, \hZf[\JX]{\Vec{\uV}}{\Vec{\uV}} \rangle
  \right|
  +
  \left\|
    \hZf[\JX]{\Vec{\uV}}{\Vec{\uV}}
    - \langle \Vec{\uV}, \hZf[\JX]{\Vec{\uV}}{\Vec{\uV}} \rangle \Vec{\uV}
  \right\|_{2}
  \\
  &\dCmt{\(  \because \| \Vec{\uV} \|_{2} = 1  \)}
  \\
  &=
  \Dxu + \Dxxu
  \\
  &\dCmt{by the definitions of the random variables \(  \Dxu, \Dxxu  \)}
\end{align*}
%|<<|===========================================================================================|<<|
\end{proof}
%|<<|~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~|<<|
%|<<|~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~|<<|
%|<<|~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~|<<|

==> results-15-2-a.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Main Result}        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\label{section:main-results} %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\THEOREM \ref{thm:adversarial}, below,
states the main result of this work, which establishes the convergence of \BIHT
when an arbitrary choice but bounded number of responses are corrupted.
%
Note that it is a universal result in the sense that the measurement matrix, \(  \Mat{\AM}  \),
is fixed across the recovery of all \ksparserealunit vectors.

%|>>|*******************************************************************************************|>>|
%|>>|*******************************************************************************************|>>|
%|>>|*******************************************************************************************|>>|
\begin{theorem}
\label{thm:adversarial}
%
Let
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \epsilonX, \errorO, \tauX \in ( 0,1 ]  \),
\(  \rX > 0  \),
\(  \k, \m, \n \in \Z_{+}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
where
%|>>|===========================================================================================|>>|
\begin{gather}
  \label{eqn:thm:adversarial:r}
  \rX \defeq
  \rXValue
  %\frac{\cX{}}{\cX{2}} \left( \rXValueX \right)
  %\frac{\cX{4} \cX{} \tauX \sqrt{\Log( \Tfrac{2e}{\tauX} )}}{\cX{2}+\cX{3}}
  ,\\ \label{eqn:thm:adversarial:epsilon_0}
  \epsilonO \defeq
  \epsilonX  + \rX
%  =
%  \epsilonX  + \frac{( 1+\qX ) \cX{4} \cX{} \tauX \sqrt{\Log( \Tfrac{2e}{\tauX} )}}{\cX{2}+\cX{3}}
,\end{gather}
%|<<|===========================================================================================|<<|
and where
%|>>|===========================================================================================|>>|
\begin{gather}
  \label{eqn:thm:adversarial:m_0}
  \m
  \geq
  \frac{4\bC\cX{}}{\epsilonX}
  \Log(
    \binom{\n}{\k}^{2}
    \binom{\n}{2\k}
    \left( \frac{12 \bC}{\epsilonX} \right)^{2\k}
    \left( \frac{3 \aC}{\rhoX} \right)
  )
  =
  \BigO(
    \frac{\k}{\epsilonX} \Log( \frac{\n}{\epsilonX \k} )
    +
    \frac{1}{\epsilonX} \Log( \frac{1}{\rhoX} )
  )
.\end{gather}
%|<<|===========================================================================================|<<|
%and where
%%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
%\(  \m \geq 4 \cX{} \mO[\epsilonO-\rX]  \).
%%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
Fix an \(  \m \times \n  \) measurement matrix,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Mat{\AM} \in \R^{\m \times \n}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
whose rows,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Vec{\AV}\VL{1}, \dots, \Vec{\AV}\VL{\m} \sim \N( \Vec{0}, \Id{\n} )  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
are \iid Gaussian random vectors, and let
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \f : \R^{\n} \to \BinarySet^{\m}  \)
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
be a map which satisfies
%|>>|===========================================================================================|>>|
\begin{gather}
\label{eqn:thm:adversarial:3}
  \DistH{\f( \Vec{\x} )}{\Sign( \Mat{\AM} \Vec{\x} )} \leq \tauX \m
\end{gather}
%|<<|===========================================================================================|<<|
for all \(  \Vec{\x} \in \R^{\n}  \).
%
Uniformly with probability at least
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  1 - \rhoX  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
for all \ksparserealunit vectors,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Vec{\x} \in \SparseSphereSubspace{\k}{\n}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
when given \(  \m  \) adversarially corrupted responses,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Vec{\yV} = \f( \Vec{\x} ) \in \BinarySet^{\m}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%with any choice of up to \(  \tauX \m  \) corrupted,
the sequence of approximations,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \{ \Vec{\xApprox}\IL{\Iter} \in \SparseSphereSubspace{\k}{\n} \}_{\Iter \in \Z_{\geq 0}}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
produced by the \NBIHT algorithm converges as
%|>>|===========================================================================================|>>|
\begin{subequations}
\label{eqn:thm:adversarial:4}
\begin{gather}
\label{eqn:thm:adversarial:4:1}
  \DistS{\Vec{\x}}{\Vec{\xApprox}\IL{\Iter}}
  \leq
  2^{2^{-\Iter}}
  \epsilonO^{1-2^{-\Iter}}
\end{gather}
%|<<|===========================================================================================|<<|
with an approximation error asymptotically bounded from above by
%|>>|===========================================================================================|>>|
\begin{gather}
\label{eqn:thm:adversarial:4:2}
  \lim_{\Iter \to \infty} \DistS{\Vec{\x}}{\Vec{\xApprox}\IL{\Iter}}
  \leq
  \epsilonO
.\end{gather}
\end{subequations}
%|<<|===========================================================================================|<<|
\end{theorem}
%|<<|*******************************************************************************************|<<|
%|<<|*******************************************************************************************|<<|
%|<<|*******************************************************************************************|<<|

\begin{comment}
%|>>|*******************************************************************************************|>>|
%|>>|*******************************************************************************************|>>|
%|>>|*******************************************************************************************|>>|
\begin{theorem}
\label{thm:adversarial}
%
Fix
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \epsilonX, \errorO, \tauX \in ( 0,1 ]  \),
\(  \rX, \qX > 0  \),
\(  \k, \m, \mO[\epsilonO-\rX], \n \in \Z_{+}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
where
%|>>|===========================================================================================|>>|
\begin{gather}
  \label{eqn:thm:adversarial:r}
  \rX \defeq
  \frac{\cX{4} \cX{} \tauX \sqrt{\Log( \Tfrac{2e}{\tauX} )}}{\cX{2}+\cX{3}}
  ,\\ \label{eqn:thm:adversarial:epsilon_0}
  \epsilonO \defeq
  \epsilonX  + ( 1+\qX ) \rX
  =
  \epsilonX  + \frac{( 1+\qX ) \cX{4} \cX{} \tauX \sqrt{\Log( \Tfrac{2e}{\tauX} )}}{\cX{2}+\cX{3}}
  ,\\ \\ \label{eqn:thm:adversarial:m_0}
  \mO[\epsilonO-\rX]
  =
  \frac{\bC}{\epsilonO-\rX}
  \Log(
    \binom{\n}{\k}^{2}
    \binom{\n}{2\k}
    \left( \frac{12 \bC}{\epsilonO-\rX} \right)^{2\k}
    \left( \frac{3 \aC}{\rhoX} \right)
  )
  =
  \BigO(
    \frac{\k}{\epsilonO-\rX} \Log( \frac{\n}{( \epsilonO-\rX ) \k} )
    +
    \frac{1}{\epsilonO-\rX} \Log( \frac{1}{\rhoX} )
  )
,\end{gather}
%|<<|===========================================================================================|<<|
and where
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \m \geq 4 \cX{} \mO[\epsilonO-\rX]  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
Fix an \(  \m \times \n  \) measurement matrix,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Mat{\AM} \in \R^{\m \times \n}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
whose rows,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Vec{\AV}\VL{1}, \dots, \Vec{\AV}\VL{\m} \sim \N( \Vec{0}, \Id{\n} )  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
are \iid Gaussian random vectors.
%
Uniformly with probability at least
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  1 - \rhoX  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
for all \ksparserealunit vectors,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Vec{\x} \in \SparseSphereSubspace{\k}{\n}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
when given \(  \m  \) noisy responses
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Vec{\yV} = \f( \Vec{\x} ) \in \BinarySet^{\m}  \)
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
with any choice of at most \(  \tauX \m  \) corrupted, such that
%|>>|===========================================================================================|>>|
\begin{gather}
\label{eqn:thm:adversarial:3}
  \DistH{\Sign( \Mat{\AM} \Vec{\x} )}{\Vec{\yV}} \leq \tauX \m
,\end{gather}
%|<<|===========================================================================================|<<|
the sequence of approximations,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \{ \Vec{\xApprox}\IL{\Iter} \in \SparseSphereSubspace{\k}{\n} \}_{\Iter \in \Z_{\geq 0}}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
produced by the \NBIHT algorithm converges as
%|>>|===========================================================================================|>>|
\begin{subequations}
\label{eqn:thm:adversarial:4}
\begin{gather}
\label{eqn:thm:adversarial:4:1}
  \DistS{\Vec{\x}}{\Vec{\xApprox}\IL{\Iter}}
  \leq
  2^{2^{-\Iter}}
  \epsilonO^{1-2^{-\Iter}}
\end{gather}
%|<<|===========================================================================================|<<|
with an approximation error asymptotically bounded from above by
%|>>|===========================================================================================|>>|
\begin{gather}
\label{eqn:thm:adversarial:4:2}
  \lim_{\Iter \to \infty} \DistS{\Vec{\x}}{\Vec{\xApprox}\IL{\Iter}}
  \leq
  \epsilonO
.\end{gather}
\end{subequations}
%|<<|===========================================================================================|<<|
\end{theorem}
%|<<|*******************************************************************************************|<<|
%|<<|*******************************************************************************************|<<|
%|<<|*******************************************************************************************|<<|

%|>>|*******************************************************************************************|>>|
%|>>|*******************************************************************************************|>>|
%|>>|*******************************************************************************************|>>|
\begin{theorem}
\label{thm:adversarial:small-tau}
%
Consider the notations and conditions of \THEOREM \ref{thm:adversarial},
and suppose
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \epsilonX
    > \rX
    = \frac{\cX{4}\cX{}}{( \cX{2}+\cX{3} ) }\, \tauX \sqrt{\Log( \Tfrac{2e}{\tauX} )}  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
%Let
%%|>>|===========================================================================================|>>|
%\begin{gather}
%\label{eqn:thm:adversarial:epsilon-approx:epsilon_0}
%  \epsilonOX
%  \defeq
%  \epsilonX - \rX
%  =
%  \epsilonX - \frac{\cX{4} \cX{}}{( \cX{2} + \cX{3} ) } \, \tauX \sqrt{\Log( \Tfrac{2e}{\tauX} )}
%  %\frac{( \cX{2} + \cX{3} ) }{\cX{}} \tauX \sqrt{16\pi \Log( \Tfrac{2e}{\tauX} )}
%  \lesssim
%  \epsilonX - 176.4978 \, \tauX \sqrt{\Log( \Tfrac{2e}{\tauX} )}
%\end{gather}
%%|<<|===========================================================================================|<<|
%and
%
Fix
%|>>|===========================================================================================|>>|
\begin{gather}
\label{eqn:thm:adversarial:epsilon-approx:m'_0}
  \mO[\epsilonX-\rX]
  =
  \frac{\bC}{\epsilonX-\rX}
  \Log(
    \binom{\n}{\k}^{2}
    \binom{\n}{2\k}
    \left( \frac{12 \bC}{\epsilonX-\rX} \right)^{2\k}
    \left( \frac{3 \aC}{\rhoX} \right)
  )
  =
  \BigO(
    \frac{\k}{\epsilonX-\rX} \Log( \frac{\n}{( \epsilonX-\rX ) \k} )
    +
    \frac{1}{\epsilonX-\rX} \Log( \frac{1}{\rhoX} )
  )
\end{gather}
%|<<|===========================================================================================|<<|
%
Suppose
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \m \geq 4\cX{} \mO[\epsilonX-\rX]  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
Uniformly with probability at least
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  1 - \rhoX  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
for all \ksparserealunit vectors,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Vec{\x} \in \SparseSphereSubspace{\k}{\n}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
the sequence of approximations,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \{ \Vec{\xApprox}\IL{\Iter} \in \SparseSphereSubspace{\k}{\n} \}_{\Iter \in \Z_{\geq 0}}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
produced by the \NBIHT algorithm converges as
%|>>|===========================================================================================|>>|
\begin{subequations}
\label{eqn:thm:adversarial:4}
\begin{gather}
\label{eqn:thm:adversarial:4:1}
  \DistS{\Vec{\x}}{\Vec{\xApprox}\IL{\Iter}}
  \leq
  2^{2^{-\Iter}}
  \epsilonX^{1-2^{-\Iter}}
\end{gather}
%|<<|===========================================================================================|<<|
with an approximation error asymptotically bounded from above by
%|>>|===========================================================================================|>>|
\begin{gather}
\label{eqn:thm:adversarial:4:2}
  \lim_{\Iter \to \infty} \DistS{\Vec{\x}}{\Vec{\xApprox}\IL{\Iter}}
  \leq
  \epsilonX
.\end{gather}
\end{subequations}
%|<<|===========================================================================================|<<|
\end{theorem}
%|<<|*******************************************************************************************|<<|
%|<<|*******************************************************************************************|<<|
%|<<|*******************************************************************************************|<<|
\end{comment}

==> technical-0-15-3.tex <==
\let\oldXu\Xu
\let\oldYu\Yu
\let\oldyu\yu
\renewcommand{\Xu}{\RV{X}_{\Vec{\uV}}}
\renewcommand{\Yu}{\Vec{Y}_{\Vec{\uV}}}
\renewcommand{\yu}{\Vec{y}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Proof of the Main Technical Theorem (\THEOREM \ref{thm:raic:adv})}
\label{section:|>pf-main-technical}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\ToDo{The function \(  \hf{}{}  \) needs to be negated throughout.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Discussion and Preliminaries}   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\label{section:|>pf-main-technical|>prelim} %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We begin by introducing and verifying some results that will set us up for
proving the main technical theorem, \THEOREM \ref{thm:raic:adv}.
%
Throughout \SECTIONS \ref{section:|>pf-main-technical}-\ref{section:|>D2},
the function
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \f : \R^{\n} \to \BinarySet^{\m}  \)
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
is taken to be any function which upholds:
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \DistH{\f( \Vec{w} )}{\Sign( \Mat{\ZX} \Vec{w} )} \leq \tauX \m  \)
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
at every point, \(  \Vec{w} \in \R^{\n}  \).
%
Specification of this condition will be henceforth omitted to avoid redundancy.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\par %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
First off, the \LHS of \EQUATION \eqref{eqn:thm:raic:adv:1} in \THEOREM \ref{thm:raic:adv},
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \left\| ( \Vec{\xV} - \Vec{\yV} ) - \hZf[\JX]{\Vec{\xV}}{\Vec{\yV}} \right\|_{2}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
is split into two components (with bounding).

%|>>|*******************************************************************************************|>>|
%|>>|*******************************************************************************************|>>|
%|>>|*******************************************************************************************|>>|
\begin{claim}
\label{claim:raic:adv:1}
%
For all
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Vec{\xV}, \Vec{\yV} \in \R^{\n}  \) and
\(  \JX \subseteq [\n]  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
the following inequality (deterministically) holds:
%|>>|===========================================================================================|>>|
\begin{align}
  \left\| ( \Vec{\xV} - \Vec{\yV} ) - \hZf[\JX]{\Vec{\xV}}{\Vec{\yV}} \right\|_{2}
  &\leq
  \left\| ( \Vec{\xV} - \Vec{\yV} ) - \hZ[\JX]( \Vec{\xV}, \Vec{\yV} )  \right\|_{2}
  +
  \left\| \hZf[\JX]{\Vec{\xV}}{\Vec{\xV}} \right\|_{2}
\label{eqn:claim:raic:adv:1:1}
.\end{align}
%|<<|===========================================================================================|<<|
\end{claim}
%|<<|*******************************************************************************************|<<|
%|<<|*******************************************************************************************|<<|
%|<<|*******************************************************************************************|<<|

%|>>|~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~|>>|
%|>>|~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~|>>|
%|>>|~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~|>>|
\begin{proof}
{\CLAIM \ref{claim:raic:adv:1}}
%
Fix
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Vec{\xV}, \Vec{\yV} \in \R^{\n}  \) and
\(  \JX \subseteq [\n]  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
arbitrarily.
%
The (random) vector
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(
  {( \Vec{\xV} - \Vec{\yV} ) - \hZf[\JX]{\Vec{\xV}}{\Vec{\yV}}}
%  =
%  {\bigl( ( \Vec{\xV} - \Vec{\yV} ) - \hZ[\JX]( \Vec{\xV}, \Vec{\yV} ) \bigr)}
%  +
%  {\bigl( \hZ[\JX]( \Vec{\xV}, \Vec{\yV} ) - \hZf[\JX]{\Vec{\xV}}{\Vec{\yV}} \bigr)}
\)
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
can be rewritten as follows:
%|>>|===========================================================================================|>>|
\begin{align*}
  ( \Vec{\xV} - \Vec{\yV} ) - \hZf[\JX]{\Vec{\xV}}{\Vec{\yV}}
  =
  \bigl( ( \Vec{\xV} - \Vec{\yV} ) - \hZ[\JX]( \Vec{\xV}, \Vec{\yV} ) \bigr)
  -
  \bigl( \hZf[\JX]{\Vec{\xV}}{\Vec{\yV}} - \hZ[\JX]( \Vec{\xV}, \Vec{\yV} ) \bigr)
,\end{align*}
%|<<|===========================================================================================|<<|
where the second and fourth terms on the \RHS cancel.
%
Additionally, observe:
%|>>|===========================================================================================|>>|
\begin{align*}
  &
  \hZf[\JX]{\Vec{\xV}}{\Vec{\yV}} - \hZ[\JX]( \Vec{\xV}, \Vec{\yV} )
  \\
  &=
  \frac{\sqrt{2\pi}}{\m}
  \sum_{\iIx=1}^{\m}
  \ThresholdSet[{\Supp( \Vec{\xV} ) \cup \Supp( \Vec{\yV} ) \cup}]{\JX}( \Vec{\ZX}\VL{\iIx} )
  \cdot
  \frac{1}{2}
  \bigl(
    \fZix
    -
    \Sign.( \langle \Vec{\yV}, \Vec{\ZX}\VL{\iIx} \rangle )
  \bigr)
  \\ &\AlignSp
  -
  \frac{\sqrt{2\pi}}{\m}
  \sum_{\iIx=1}^{\m}
  \ThresholdSet[{\Supp( \Vec{\xV} ) \cup \Supp( \Vec{\yV} ) \cup}]{\JX}( \Vec{\ZX}\VL{\iIx} )
  \cdot
  \frac{1}{2}
  \bigl(
    \Sign.( \langle \Vec{\xV}, \Vec{\ZX}\VL{\iIx} \rangle )
    -
    \Sign.( \langle \Vec{\yV}, \Vec{\ZX}\VL{\iIx} \rangle )
  \bigr)
  \\
  &=
  \frac{\sqrt{2\pi}}{\m}
  \sum_{\iIx=1}^{\m}
  \ThresholdSet[{\Supp( \Vec{\xV} ) \cup \Supp( \Vec{\yV} ) \cup}]{\JX}( \Vec{\ZX}\VL{\iIx} )
  \cdot
  \frac{1}{2}
  \Bigl(
  \bigl(
    \fZix
    -
    \Sign.( \langle \Vec{\yV}, \Vec{\ZX}\VL{\iIx} \rangle )
  \bigr)
  -
  \bigl(
    \Sign.( \langle \Vec{\xV}, \Vec{\ZX}\VL{\iIx} \rangle )
    -
    \Sign.( \langle \Vec{\yV}, \Vec{\ZX}\VL{\iIx} \rangle )
  \bigr)
  \Bigr)
  \\
  &=
  \frac{\sqrt{2\pi}}{\m}
  \sum_{\iIx=1}^{\m}
  \ThresholdSet[{\Supp( \Vec{\xV} ) \cup \Supp( \Vec{\yV} ) \cup}]{\JX}( \Vec{\ZX}\VL{\iIx} )
  \cdot
  \frac{1}{2}
  \bigl(
    \fZix
    -
    \Sign.( \langle \Vec{\xV}, \Vec{\ZX}\VL{\iIx} \rangle )
  \bigr)
  \\
  &=
  \hZf[\JX]{\Vec{\xV}}{\Vec{\xV}}
\end{align*}
%|<<|===========================================================================================|<<|
%
Thus, combining above work:
%|>>|===========================================================================================|>>|
\begin{align*}
  ( \Vec{\xV} - \Vec{\yV} ) - \hZf[\JX]{\Vec{\xV}}{\Vec{\yV}}
  &=
  \bigl( ( \Vec{\xV} - \Vec{\yV} ) - \hZ[\JX]( \Vec{\xV}, \Vec{\yV} ) \bigr)
  -
  \bigl( \hZf[\JX]{\Vec{\xV}}{\Vec{\yV}} - \hZ[\JX]( \Vec{\xV}, \Vec{\yV} ) \bigr)
  \\
  &=
  \bigl( ( \Vec{\xV} - \Vec{\yV} ) - \hZ[\JX]( \Vec{\xV}, \Vec{\yV} ) \bigr)
  - \hZf[\JX]{\Vec{\xV}}{\Vec{\xV}}
.\end{align*}
%|<<|===========================================================================================|<<|
%
Then, the norm is upper bounded as follows:
%|>>|===========================================================================================|>>|
\begin{align*}
  \left\| ( \Vec{\xV} - \Vec{\yV} ) - \hZf[\JX]{\Vec{\xV}}{\Vec{\yV}} \right\|_{2}
  &=
  \left\|
    \bigl( ( \Vec{\xV} - \Vec{\yV} ) - \hZ[\JX]( \Vec{\xV}, \Vec{\yV} ) \bigr)
    - \hZf[\JX]{\Vec{\xV}}{\Vec{\xV}}
  \right\|_{2}
  \\
  &\leq
  \left\| ( \Vec{\xV} - \Vec{\yV} ) - \hZ[\JX]( \Vec{\xV}, \Vec{\yV} ) \right\|_{2}
  +
  \left\| \hZf[\JX]{\Vec{\xV}}{\Vec{\xV}} \right\|_{2}
\end{align*}
%|<<|===========================================================================================|<<|
where the bottom line applies the triangle inequality.
\end{proof}
%|<<|~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~|<<|
%|<<|~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~|<<|
%|<<|~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~|<<|

\EQUATION* \eqref{eqn:claim:raic:adv:1:1} of \CLAIM \ref{claim:raic:adv:1}
decomposes (with bounding) the random variable of interest,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \left\| ( \Vec{\xV} - \Vec{\yV} ) - \hZf[\JX]{\Vec{\xV}}{\Vec{\yV}} \right\|_{2}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
into two terms which are individually easier to control.
%
The majority of the argument for \THEOREM \ref{thm:raic:adv} is towards
a uniform upper bound on the latter term of this decomposition,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \DXX{\Vec{\xV}}{\Vec{\xV}} \defeq
    \left\| \hZf[\JX]{\Vec{\xV}}{\Vec{\xV}} \right\|_{2}  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
This second term, \(  \DXX{\Vec{\xV}}{\Vec{\xV}}  \), requires new analysis,
which takes up \SECTIONS \ref{section:|>pf-main-technical|>prelim|>D2} and \ref{section:|>D2}.
%
On the other hand, the first term,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \DX{\Vec{\xV}}{\Vec{\xV}} \defeq
    \left\| ( \Vec{\xV} - \Vec{\yV} ) - \hZ[\JX]( \Vec{\xV}, \Vec{\yV} ) \right\|_{2}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
is immediately upper bounded with high probability for all
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Vec{\xV}, \Vec{\yV} \in \SparseSphereSubspace{\k}{\n}  \)
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
via \cite[\THEOREM 3.3]{matsumoto2022binary}, stated below.

%|>>|*******************************************************************************************|>>|
%|>>|*******************************************************************************************|>>|
%|>>|*******************************************************************************************|>>|
\begin{lemma}[{\cite[\THEOREM 3.3]{matsumoto2022binary}}]
\label{lemma:raic-for-gaussians}
%
Fix
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \epsilonRAIC, \rhoRAIC \in (0,1)  \),
\(  \k, \m, \n \in \Z_{+}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
such that
%|>>|===========================================================================================|>>|
\begin{gather}
\label{eqn:lemma:raic-for-gaussians:1}
  \m \geq
  \frac{\bC}{\epsilonRAIC}
  \Log(
    \binom{\n}{\k}^{2}
    \binom{\n}{2\k}
    \left( \frac{12 \bC}{\epsilonRAIC} \right)^{2\k}
    \left( \frac{\aC}{\rhoRAIC} \right)
  )
%  \in
%  \BigO(
%    \frac{\k}{\epsilonX}
%    \Log( \frac{\n}{\epsilonX \k} )
%    +
%    \frac{1}{\epsilonX}
%    \Log( \frac{1}{\rhoX} )
%  )
.\end{gather}
%|<<|===========================================================================================|<<|
%
Then, uniformly with probability at least
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  1 - \rhoRAIC  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
the Gaussian measurement matrix \(  \Mat{\AM} \in \R^{\m \times \n}  \) satisfies the
\(  ( \k, \n, \epsilonRAIC, \cX{1}, \cX{2} )  \)-RAIC:
%|>>|===========================================================================================|>>|
\begin{gather}
\label{eqn:lemma:raic-for-gaussians:2}
  \bigl\| ( \Vec{x} - \Vec{y} ) - \h[\JX]( \Vec{x}, \Vec{y} ) \bigr\|_{2}
  \leq
  \cX{1} \sqrt{\epsilonRAIC \DistS{\Vec{x}}{\Vec{y}}} + \cX{2} \epsilonRAIC
\end{gather}
%|<<|===========================================================================================|<<|
for all
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Vec{x}, \Vec{y} \in \SparseSphereSubspace{\k}{\n}  \) and all
\(  \JX \subseteq [\n]  \), \(  | \JX | \leq \k  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
\end{lemma}
%|<<|*******************************************************************************************|<<|
%|<<|*******************************************************************************************|<<|
%|<<|*******************************************************************************************|<<|

%On the other hand, the second term, \(  \DXX{\Vec{\xV}}{\Vec{\xV}}  \),
%in \EQUATION \eqref{eqn:claim:raic:adv:1:1} requires new analysis,
%which takes up \SECTIONS \ref{section:|>pf-main-technical|>prelim|>D2} and \ref{section:|>D2}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Discussion Regarding \texorpdfstring{\( \DXX{\Vec{\xV}}{\Vec{\xV}} \)}{D2;J(x,x)}} %%
\label{section:|>pf-main-technical|>prelim|>D2}                                                   %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%>
%\COMMENT{This section needs work.. Notations are overly complicated (also inconsistent..). Will fix this up soon.}

The derivation of an upper bound on the random variable,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \DXX{\Vec{\xV}}{\Vec{\xV}} = \| \hZf[\JX]{\Vec{\xV}}{\Vec{\xV}} \|_{2}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
will entirely ignore the specification of the vector \(  \Vec{\xV}  \).
%
Rather, recall the definition of \(  \hZf[\JX]{}{}  \):
%|>>|===========================================================================================|>>|
\begin{align*}
  \hZf[\JX]{\Vec{w}}{\Vec{w'}}
  &=
  \frac{\sqrt{2\pi}}{\m}
  \sum_{\iIx=1}^{\m}
  \TJZi
  \cdot \frac{1}{2}
  \left( \Big.
    \f( \Vec{w} )_{\iIx}
    -
    \Sign( \langle \Vec{w'}, \Vec{\ZX}\VL{\iIx} \rangle )
  \right)
  \\
  &=
  \frac{\sqrt{2\pi}}{\m}
  \sum_{\iIx=1}^{\m}
  \TJZi
  \cdot \frac{1}{2}
  \left( \Big.
    \f( \Vec{w} )
    -
    \Sign( \Mat{\ZX} \Vec{w'} )
  \right)_{\iIx}
\end{align*}
%|<<|===========================================================================================|<<|
where
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Mat{\ZX} \in \R^{\m \times \n}  \),
\(  \Mat{\ZX} = ( \Vec{\ZX}\VL{1} \;\cdots\; \Vec{\ZX}\VL{\m} )^{\T}  \), and where
\(  \Vec{w}, \Vec{w'} \in \R^{\n}  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
The only dependence of \(  \hZf[\JX]{\Vec{w}}{\Vec{w'}}  \) on the preimage,
\(  ( \Vec{w}, \Vec{w'} )  \), is captured in the expression:
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \f( \Vec{w} ) - \Sign( \Mat{\ZX} \Vec{w'} )  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
where the images of \(  \f  \) and \(  \Sign  \) over \(  \R^{\n}  \) and \(  \R^{\m}  \),
respectively, are subsets of the set
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \{ \Vec{z} \in \{ -1,0,1 \}^{\m} : \| \Vec{z} \|_{0} \leq \tauX \m \}  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
All else is fixed across all \(  ( \Vec{w}, \Vec{w'} ) \in \R^{\m} \times \R^{\m}  \).
%
Thus, upon fixing the set of Gaussian vectors, \(  \Mat{\AV}\VL{1}, \dots, \Mat{\AV}\VL{\m}  \),
for each
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \JX \subseteq [\n]  \), \(  | \JX | \leq \kX  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
the image of the function \(  \hZf[\JX]{}{}  \) has finite cardinality no more than:
%|>>|===========================================================================================|>>|
\begin{gather*}
  \left|
    \hZf[\JX]{}{} \left[ \PREIMG \right]
  \right|
  \leq
  %\sum_{\Ell=1}^{\kX} \binom{\n}{\Ell}
  \sum_{\Ell=1}^{\tauX \m} \binom{\m}{\Ell} 2^{\Ell}
%  \leq
%  %4 \binom{\n}{\kX}
%  4 \cdot 2^{\tauX \m} \binom{\m}{\tauX \m}
.\end{gather*}
%|<<|===========================================================================================|<<|
%
It then suffices to enumerate each of the up to
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \sum_{\Ell=1}^{\tauX \m} \binom{\m}{\Ell} 2^{\Ell}  \)-many
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
vectors comprising
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \hZf[\JX]{}{} \left[ \PREIMG \right]  \)
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
and bound their norms for each choice of \(  \JX \subseteq [\n]  \), \(  | \JX | \leq \kX  \).
%
With this motivation, construct a collection of sets,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \US[\JX] \subseteq \SparseSphereSubspace{\k}{\n}  \), \(  \JX \subseteq [\n]  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
by inserting precisely one vector,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Vec{\uV} \in \SparseSphereSubspace{\k}{\n}  \),
%\(  \Supp( \Vec{\uV} ) \subseteq \JX  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
into \(  \US[\JX]  \) for each vector \(  \Vec{z} \in \hZf[\JX]{}{} \left[ \PREIMG \right]  \)
such that
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \hZf[\JX]{\Vec{\uV}}{\Vec{\uV}} = \Vec{z}  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
%For later use, additionally define the set
%%|>>|===========================================================================================|>>|
%\begin{gather}
%  \US = \bigcup_{\substack{\JX \subseteq [\n] :\\ | \JX | \leq \kX}} \US[\JX]
%.\end{gather}
%%|<<|===========================================================================================|<<|
%
The above discussion is formalized and verified in the following claim and its proof.

%|>>|*******************************************************************************************|>>|
%|>>|*******************************************************************************************|>>|
%|>>|*******************************************************************************************|>>|
\begin{claim}
\label{claim:raic:adv:2}
%
Fix
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \gamma \geq 0  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
Suppose for all
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \JX \subseteq [\n]  \), \(  | \JX | \leq \kX  \), and
\(  \Vec{\uV} \in \US[\JX]  \), %\(  \Supp( \Vec{\uV} ) \subseteq \JX  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
the norm of \(  \hZf[\JX]{\Vec{\uV}}{\Vec{\uV}}  \) is bounded from above by:
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \| \hZf[\JX]{\Vec{\uV}}{\Vec{\uV}} \|_{2} \leq \gamma  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
Then, uniformly for all \(  \Vec{\xV} \in \SparseSphereSubspace{\k}{\n}  \) and
for all \(  \JX \subseteq [\n]  \), \(  | \JX | \leq \kX  \),
the same bound holds at \(  ( \Vec{\xV}, \Vec{\xV} )  \):
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \| \hZf[\JX]{\Vec{\xV}}{\Vec{\xV}} \|_{2} \leq \gamma  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
\end{claim}
%|<<|*******************************************************************************************|<<|
%|<<|*******************************************************************************************|<<|
%|<<|*******************************************************************************************|<<|

%|>>|~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~|>>|
%|>>|~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~|>>|
%|>>|~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~|>>|
\begin{proof}
{\CLAIM \ref{claim:raic:adv:2}}
%
Suppose for the sake of contradiction that
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \| \hZf[\JX]{\Vec{\uV}}{\Vec{\uV}} \|_{2} \leq \gamma  \)
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
for each
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \JX \subseteq [\n]  \), \(  | \JX | \leq \kX  \), and
\(  \Vec{\uV} \in \US[\JX]  \), %\(  \Supp( \Vec{\uV} ) \subseteq \JX  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
but there exists
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Jx \subseteq [\n]  \), \(  | \Jx | \leq \kX  \), and
\(  \Vec{\xV} \in \SparseSphereSubspace{\k}{\n}  \), %\(  \Supp( \Vec{\xV} ) \subseteq \Jx  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
for which
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \| \hZf[\Jx]{\Vec{\xV}}{\Vec{\xV}} \|_{2} > \gamma  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
Denote the image of \(  ( \Vec{\xV}, \Vec{\xV} )  \) under \(  \hZf[\Jx]{}{}  \) by
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Vec{z} = \hZf[\Jx]{\Vec{\xV}}{\Vec{\xV}}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
where by assumption,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \| \Vec{z} \|_{2} > \gamma  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
and let
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(
  \Set{\WX} =
  \{ \Vec{\wV} \in \SparseSphereSubspace{\k}{\n} : \hZf[\Jx]{\Vec{\wV}}{\Vec{\wV}} = \Vec{\zV} \}
\).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
Then, by the construction of the set \(  \US[\Jx]  \), it must be that
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  | \US[\Jx] \cap \Set{\WX} | = 1  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%there is precisely one vector
%\(  \Vec{\wV} \in \Set{\WX}  \) from the set \(  \Set{\WX}  \) such that
%\(  \Vec{\wV} \in \US[\Jx]  \),
which implies that there exists
\(  \Vec{\uV} \in \US[\Jx]  \) for which
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \| \hZf[\JX]{\Vec{\uV}}{\Vec{\uV}} \|_{2} = \| \Vec{z} \|_{2} > \gamma  \)%
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
---a contradiction.
%
By this contradiction, the claim holds.
\end{proof}
%|<<|~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~|<<|
%|<<|~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~|<<|
%|<<|~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~|<<|

Due \CLAIM \ref{claim:raic:adv:2},
the proof of \THEOREM \ref{thm:raic:adv} will seek to bound
\(  \| \hZf[\JX]{\Vec{\uV}}{\Vec{\uV}} \|_{2}  \) from above for all
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \JX \subseteq [\n]  \), \(  | \JX | \leq \kX  \), and \(  \Vec{\uV} \in \US[\JX]  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
Specifically, \LEMMA \ref{lemma:D2} controls this random variable,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \DXX{\Vec{\uV}}{\Vec{\uV}} = \| \hZf[\JX]{\Vec{\uV}}{\Vec{\uV}} \|_{2}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
uniformly for every
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \JX \subseteq [\n]  \), \(  | \JX | \leq \kX  \), and \(  \Vec{\uV} \in \US[\JX]  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|

%|>>|*******************************************************************************************|>>|
%|>>|*******************************************************************************************|>>|
%|>>|*******************************************************************************************|>>|
\begin{lemma}
\label{lemma:D2}
%
Let \(  \m \in \Z_{+}  \) satisfy
%|>>|===========================================================================================|>>|
\begin{gather*}
  m
  \geq
  \frac{\bC}{\epsilonRAICadv}
  \Log(
    \binom{\n}{\k}^{2}
    \binom{\n}{2\k}
    \left( \frac{12 \bC}{\epsilonRAICadv} \right)^{2\k}
    \left( \frac{3 \aC}{\rhoX} \right)
  )
  =
  \BigO(
    \frac{\k}{\epsilonRAICadv} \Log( \frac{\n}{\epsilonRAICadv \k} )
    +
    \frac{1}{\epsilonRAICadv} \Log( \frac{1}{\rhoX} )
  )
.\end{gather*}
%|<<|===========================================================================================|<<|
%
With probability at least
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  1 - \frac{2\rhoX}{3}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
uniformly for all
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \JX \subseteq [\n]  \), \(  | \JX | \leq \k  \), and \(  \Vec{\uV} \in \US[\JX]  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%|>>|===========================================================================================|>>|
\begin{gather}
  \DXXu \leq \DXXuUB = \DXXuUBconst
%  \leq
%  13\sqrt{\frac{\pi \epsilonRAICadv \tauX}{\bC}}
%  +
%  \left( 2 + 4\sqrt{\pi} \right) \tauX \sqrt{\Log( \Tfrac{2e}{\tauX} )}
.\end{gather}
%|<<|===========================================================================================|<<|
\end{lemma}
%|<<|*******************************************************************************************|<<|
%|<<|*******************************************************************************************|<<|
%|<<|*******************************************************************************************|<<|

The proof of the lemma is deferred to \APPENDIX \ref{section:|>appendix|>D2:ub}.
%
Next, \THEOREM \ref{thm:raic:adv} is proved,
contingent on the proof of \LEMMA \ref{lemma:D2}.

%|>>|~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~|>>|
%|>>|~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~|>>|
%|>>|~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~|>>|
\begin{proof}
{\THEOREM \ref{thm:raic:adv}}
%
Fix
%|>>|===========================================================================================|>>|
%\begin{gather*}
\(
  m
  =
  \frac{\bC}{\epsilonRAICadv}
  \Log*(
    \binom{\n}{\k}^{2}
    \binom{\n}{2\k}
    ( \frac{12 \bC}{\epsilonRAICadv} )^{2\k}
    ( \frac{3 \aC}{\rhoX} )
  )
\).
%.\end{gather*}
%|<<|===========================================================================================|<<|
%
Due to \CLAIM \ref{claim:raic:adv:1}, for every
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Vec{\xV}, \Vec{\yV} \in \R^{\n}  \)
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
and every
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \JX \subseteq [\n]  \), %\(  | \JX | \leq \kX  \)
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%|>>|===========================================================================================|>>|
\begin{align*}
  \left\| ( \Vec{\xV} - \Vec{\yV} ) - \hZf[\JX]{\Vec{\xV}}{\Vec{\yV}} \right\|_{2}
  &\leq
  \left\| ( \Vec{\xV} - \Vec{\yV} ) - \hZ[\JX]( \Vec{\xV}, \Vec{\yV} )  \right\|_{2}
  +
  \left\| \hZf[\JX]{\Vec{\xV}}{\Vec{\xV}} \right\|_{2}
\end{align*}
%|<<|===========================================================================================|<<|
%
By \LEMMA \ref{lemma:raic-for-gaussians} (\cite[\THEOREM 3.3]{matsumoto2022binary}),
with probability at least
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  1 - \frac{\rhoX}{3}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
uniformly for all
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Vec{\xV}, \Vec{\yV} \in \SparseSphereSubspace{\k}{\n}  \) and
\(  \JX \subseteq [\n]  \), \(  | \JX | \leq \k  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%|>>|===========================================================================================|>>|
\begin{align*}
  \left\| ( \Vec{\xV} - \Vec{\yV} ) - \hZ[\JX]( \Vec{\xV}, \Vec{\yV} )  \right\|_{2}
  \leq
  \cX{1} \sqrt{\epsilonRAICadv \DistS{\Vec{x}}{\Vec{y}}}
  +
  \cX{2} \epsilonRAICadv
,\end{align*}
%|<<|===========================================================================================|<<|
where \(  \cX{1}, \cX{2} > 0  \) are universal constants as defined in
\EQUATION \eqref{eqn:universal-constants}.
%
Additionally, by \LEMMA \ref{lemma:D2},
with probability at least
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  1 - \frac{2\rhoX}{3}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
uniformly for all
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \JX \subseteq [\n]  \), \(  | \JX | \leq \k  \), and \(  \Vec{\uV} \in \US[\JX]  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%|>>|===========================================================================================|>>|
\begin{align*}
  \left\| \hZf[\JX]{\Vec{\uV}}{\Vec{\uV}} \right\|_{2} \leq \DXXuUB = \DXXuUBconst
%  14\sqrt{\frac{\pi \epsilonRAICadv \tauX}{\bC}} + \tauX \sqrt{16\pi \Log( \Tfrac{2e}{\tauX} )}
.\end{align*}
%|<<|===========================================================================================|<<|
%
Recalling \CLAIM \ref{claim:raic:adv:2}, it follows that the same bound on
\(  \left\| \hZf[\JX]{\Vec{\xV}}{\Vec{\xV}} \right\|_{2}  \)
holds uniformly over all
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Vec{\xV} \in \SparseSphereSubspace{\k}{\n}  \),
\(  \JX \subseteq [\n]  \), \(  | \JX | \leq \kX  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
with the same probability.
%
Combining the above bounds on
\(  \left\| ( \Vec{\xV} - \Vec{\yV} ) - \hZ[\JX]( \Vec{\xV}, \Vec{\yV} )  \right\|_{2}  \) and
\(  \left\| \hZf[\JX]{\Vec{\uV}}{\Vec{\uV}} \right\|_{2}  \)
via a union bound, and applying \CLAIM \ref{claim:raic:adv:1},
the desired upper bound follows:
with probability at least
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  1 - \frac{\rhoX}{3} - \frac{2\rhoX}{3} = 1 - \rhoX  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
uniformly for all
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Vec{\xV}, \Vec{\yV} \in \SparseSphereSubspace{\k}{\n}  \),
\(  \JX \subseteq [\n]  \), \(  | \JX | \leq \kX  \):
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%|>>|===========================================================================================|>>|
\begin{align*}
  \left\| ( \Vec{\xV} - \Vec{\yV} ) - \hZf[\JX]{\Vec{\xV}}{\Vec{\yV}} \right\|_{2}
  &\leq
  \left\| ( \Vec{\xV} - \Vec{\yV} ) - \hZ[\JX]( \Vec{\xV}, \Vec{\yV} )  \right\|_{2}
  +
  \left\| \hZf[\JX]{\Vec{\xV}}{\Vec{\xV}} \right\|_{2}
  \\
  &\leq
  \cX{1} \sqrt{\epsilonRAICadv \DistS{\Vec{x}}{\Vec{y}}} + \cX{2} \epsilonRAICadv
  +
  \DXXuUB
%  14\sqrt{\frac{\pi \epsilonRAICadv \tauX}{\bC}} + \tauX \sqrt{16\pi \Log( \Tfrac{2e}{\tauX} )}
  \\
  &=
  \cX{1} \sqrt{\epsilonRAICadv \DistS{\Vec{x}}{\Vec{y}}} + \cX{2} \epsilonRAICadv
  +
  \DXXuUBconst
%  \cX{3} \sqrt{\epsilonRAICadv \tauX} + \tauX \sqrt{16\pi \Log( \Tfrac{2e}{\tauX} )}
%  \\
%  &=
%  \cX{1} \sqrt{\epsilonRAICadv \DistS{\Vec{x}}{\Vec{y}}}
%  +
%  ( \cX{2} + \cX{3} ) \epsilonRAICadv
%  +
%  \tauX \sqrt{16\pi \Log( \Tfrac{2e}{\tauX} )}
\end{align*}
%|<<|===========================================================================================|<<|
where \(  \cX{1}, \cX{2}, \cX{3}, \cX{4} > 0  \) are universal constants specified in
\EQUATION \eqref{eqn:universal-constants}.
%
%Additionally, in the case when \(  \tauX \leq \epsilonRAICadv  \),
%this is further bounded from above by:
%%|>>|===========================================================================================|>>|
%\begin{align*}
%  \left\| ( \Vec{\xV} - \Vec{\yV} ) - \hZf[\JX]{\Vec{\xV}}{\Vec{\yV}} \right\|_{2}
%  &\leq
%  \cX{1} \sqrt{\epsilonRAICadv \DistS{\Vec{x}}{\Vec{y}}}
%  +
%  ( \cX{2} + \cX{3} ) \epsilonRAICadv
%  +
%  \tauX \sqrt{16\pi \Log( \Tfrac{2e}{\tauX} )}
%.\end{align*}
%%|<<|===========================================================================================|<<|
\end{proof}
%|<<|~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~|<<|
%|<<|~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~|<<|
%|<<|~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~|<<|

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Analysis for \texorpdfstring{\(  \DXX{\Vec{\uV}}{\Vec{\uV}}  \)}{D2;J(u,u)}} %%%%%%%%%%%%%%
\label{section:|>D2}                                                                  %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\renewcommand{\Dx}[3][\JX]{\DRV'_{1;#1}( #2,#3 )}
\renewcommand{\Dxx}[3][\JX]{\DRV'_{2;#1}( #2,#3 )}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{An Orthogonal Decomposition} %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\label{section:|>D2|>ortho-decomp}       %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

To control the random variable,
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \DXX{\Vec{\uV}}{\Vec{\uV}} \defeq \| \hZf[\JX]{\Vec{\uV}}{\Vec{\uV}} \|_{2}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
the random vector, \(  \hZf[\JX]{\Vec{\uV}}{\Vec{\uV}}  \), is orthogonally decomposed into
two components:
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \langle \Vec{\uV}, \hZf[\JX]{\Vec{\uV}}{\Vec{\uV}} \rangle \Vec{\uV}  \) and
\(  \hZf[\JX]{\Vec{\uV}}{\Vec{\uV}}
    - \langle \Vec{\uV}, \hZf[\JX]{\Vec{\uV}}{\Vec{\uV}} \rangle \Vec{\uV}  \),
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
where
%|>>|===========================================================================================|>>|
\begin{gather}
  \hZf[\JX]{\Vec{\uV}}{\Vec{\uV}}
  =
  \langle \Vec{\uV}, \hZf[\JX]{\Vec{\uV}}{\Vec{\uV}} \rangle \Vec{\uV}
  +
  \bigl( \hZf[\JX]{\Vec{\uV}}{\Vec{\uV}}
         - \langle \Vec{\uV}, \hZf[\JX]{\Vec{\uV}}{\Vec{\uV}} \rangle \Vec{\uV} \bigr)
\label{eqn:raic:adv:1}
.\end{gather}
%|<<|===========================================================================================|<<|
%
As such, define the random variables, \(  \Dxu  \) and \(  \Dxxu  \), by
%|>>|===========================================================================================|>>|
\begin{gather}
  \Dxu = \left| \langle \Vec{\uV}, \hZf[\JX]{\Vec{\uV}}{\Vec{\uV}} \rangle \right|
  ,\\
  \Dxxu
  =
  \left\|
    \hZf[\JX]{\Vec{\uV}}{\Vec{\uV}}
    - \langle \Vec{\uV}, \hZf[\JX]{\Vec{\uV}}{\Vec{\uV}} \rangle \Vec{\uV}
  \right\|_{2}
\label{eqn:raic:adv:2}
.\end{gather}
%|<<|===========================================================================================|<<|

We make use of this decomposition and these random variables in the following claim.

%|>>|*******************************************************************************************|>>|
%|>>|*******************************************************************************************|>>|
%|>>|*******************************************************************************************|>>|
\begin{claim}
\label{claim:raic:adv:3}
%
For any \(  \JX \subseteq [\n]  \) and \(  \Vec{\uV} \in \R^{\n}  \),
%|>>|===========================================================================================|>>|
\begin{gather}
  \DXXu \leq \Dxu + \Dxxu
\label{eqn:raic:adv:3}
.\end{gather}
%|<<|===========================================================================================|<<|
\end{claim}
%|<<|*******************************************************************************************|<<|
%|<<|*******************************************************************************************|<<|
%|<<|*******************************************************************************************|<<|

\noindent%
Thus, \(  \DXX{\Vec{\uV}}{\Vec{\uV}}  \) can be upper bounded by bounding
\(  \Dxu  \) and \(  \Dxxu  \), the latter two of which are simpler to handle
than directly characterizing \(  \DXX{\Vec{\uV}}{\Vec{\uV}}  \).
%
Such bounds are obtained in \SECTIONS \ref{section:|>D'1} and \ref{section:|>D'2},
respectively.
%
The proof of \LEMMA \ref{lemma:D2}, which upper bounds \(  \DXX{\Vec{\uV}}{\Vec{\uV}}  \),
is deferred to \APPENDIX \ref{section:|>appendix|>D2:ub},
while the proof of \CLAIM \ref{claim:raic:adv:3} is provided in
\APPENDIX \ref{section:|>pf-claim:raic:adv:3}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Concentration Inequalities for the Orthogonal Decomposition} %%%%%%%%%%%%%%%%%%%%%%%%%%%
\label{section:|>D2|>concentration-ineq}                                 %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\renewcommand{\ZX}{Z}

\let\newXu\Xu
\let\Xu\oldXu
\let\newYu\Yu
\let\Yu\oldYu

%\ToDo{The following lemmas need to be modified/rewritten to be consistent.}

Before the random variables, \(  \Dxu  \) and \(  \Dxxu  \), are bounded,
two concentration inequalities are stated below as
\LEMMAS \ref{lemma:concentration-ineq:1} and \ref{lemma:concentration-ineq:3}
to facilitate the analysis.
%
The proofs of these lemmas are deferred to \SECTION \ref{section:|>ortho-decomp}.

%|>>|*******************************************************************************************|>>|
%|>>|*******************************************************************************************|>>|
%|>>|*******************************************************************************************|>>|
\begin{lemma}
\label{lemma:concentration-ineq:1}
%
Fix
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \lu, \tu > 0  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
Let
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Set{\ZX} = \{ \Vec{\ZX}\VL{1}, \dots, \Vec{\ZX}\VL{\lu} \sim \N( \Vec{0}, \Id{\n} ) \}  \)
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
be a collection of \(  \lu  \) \iid Gaussian vectors, and fix a \ksparserealunit vector,
\(  \Vec{\uX} \in \SparseSphereSubspace{\k}{\n}  \),
and a coordinate subset, \(  \JX \subseteq [\n]  \), \(  | \JX | \leq \kX  \).
%where \(  \Supp( \Vec{\uX} ) \subseteq \JX  \).
%
Define the random variables
%|>>|===============================z============================================================|>>|
\begin{gather*}
  \Xu[\iIx] \defeq
  \left\langle \Vec{\uX}, \TJZi \right\rangle \Sign( \langle \Vec{\uV}, \TJZi \rangle )
,\end{gather*}
%|<<|===========================================================================================|<<|
for \(  \iIx \in [\lu]  \), and
%|>>|===========================================================================================|>>|
\begin{gather*}
  \barXu
  \defeq
  \left\langle
    \Vec{\uX},
    \sum_{\iIx=1}^{\lu} \TJZi \Sign( \langle \Vec{\uV}, \TJZi \rangle )
  \right\rangle
  =
  \sum_{\iIx=1}^{\lu} \Xu[\iIx]
.\end{gather*}
%|<<|===========================================================================================|<<|
%
The concentration of the random variable \(  \barXu  \) is such that
%|>>|===========================================================================================|>>|
\begin{gather}
\label{eqn:lemma:concentration-ineq:1:1}
  \Pr \left(
    \barXu \geq \left( \sqrt{\tfrac{2}{\pi}} + \tu \right) \lu
  \right)
  \leq
  e^{-\frac{1}{2} \lu \tu^{2}}
.\end{gather}
%|<<|===========================================================================================|<<|
%
Additionally, for each \(  \iIx \in [\Ell]  \), the is an equivalence:
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  | \Xu[\iIx] | = \Xu[\iIx]  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
\end{lemma}
%|<<|*******************************************************************************************|<<|
%|<<|*******************************************************************************************|<<|
%|<<|*******************************************************************************************|<<|

%|>>|*******************************************************************************************|>>|
%|>>|*******************************************************************************************|>>|
%|>>|*******************************************************************************************|>>|
\begin{lemma}
\label{lemma:concentration-ineq:3}
%
Fix
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \lu, \tu > 0  \).
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
%
Let
%|>>|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|>>|
\(  \Set{\ZX} = \{ \Vec{\ZX}\VL{1}, \dots, \Vec{\ZX}\VL{\lu} \sim \N( \Vec{0}, \Id{\n} ) \}  \)
%|<<|:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::|<<|
be a collection of \(  \lu  \) \iid Gaussian vectors, and fix a \ksparserealunit vector,
\(  \Vec{\uX} \in \SparseSphereSubspace{\k}{\n}  \),
and a coordinate subset, \(  \JX \subseteq [\n]  \), \(  | \JX | \leq \kX  \).
%where \(  \Supp( \Vec{\uX} ) \subseteq \JX  \).
%
Define the random vector
%|>>|===========================================================================================|>>|
\begin{gather*}
  \barYu =
  \sum_{\iIx=1}^{\lu}
  \Big(
    \TJZi \Sign( \langle \Vec{\uV}, \TJZi \rangle )
    -
    \langle \Vec{\uV}, \TJZi \rangle \Sign( \langle \Vec{\uV}, \TJZi \rangle ) \Vec{\uV}
  \Big)
.\end{gather*}
%|<<|===========================================================================================|<<|
%
The concentration of the random variable representing its norm, \(  \| \barYu \|_{2}  \),
is such that
%|>>|===========================================================================================|>>|
\begin{gather}
\label{eqn:lemma:concentration-ineq:3:1}
  \Pr \left(
    \left\| \barYu \right\|_{2} > \sqrt{\frac{( \kX-1 ) \lu}{2}} + \lu \tu
  \right)
  \leq
  e^{-\frac{1}{2} \lu \tu^{2}}
.\end{gather}
%|<<|===========================================================================================|<<|
\end{lemma}
%|<<|*******************************************************************************************|<<|
%|<<|*******************************************************************************************|<<|
%|<<|*******************************************************************************************|<<|

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\renewcommand{\ZX}{A}

\let\oldXu\Xu
\let\Xu\newXu
\let\oldYu\Yu
\let\Yu\newYu

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\let\Xu\oldXu
\let\Yu\oldYu
\let\yu\oldyu

\renewcommand{\Dx}{\DRV\RVL{1}}
\renewcommand{\Dxx}{\DRV\RVL{2}}
